Multipacking on graphs and Euclidean metric space

A \emph{multipacking} in an undirected graph $G=(V,E)$ is a set $M\subseteq V$ such that for every vertex $v\in V$ and for every integer $r\geq 1$, the ball of radius $ r $ around $ v $ contains at most $r$ vertices of $M$. The \textsc{Multipacking} problem asks whether a graph contains a multipacking of size at least $k$. For more than a decade, it remained open whether \textsc{Multipacking} is \textsc{NP-complete} or polynomial-time solvable, although it is known to be polynomial-time solvable for some classes (e.g., strongly chordal graphs and grids). Foucaud, Gras, Perez, and Sikora [\textit{Algorithmica} 2021] showed it is \textsc{NP-complete} for directed graphs and \textsc{W[1]-hard} when parameterized by the solution size. We resolve the open question by proving \textsc{Multipacking} is \textsc{NP-complete} for undirected graphs and \textsc{W[2]-hard} when parameterized by the solution size. Furthermore, we show it remains \textsc{NP-complete} and \textsc{W[2]-hard} even for chordal, bipartite, claw-free, regular, CONV, and chordal$\cap\frac{1}{2}$-hyperbolic graphs (a superclass of strongly chordal graphs), and we provide approximation algorithms for cactus, chordal, and $\delta$-hyperbolic graphs. Moreover, we study the relationship between multipacking number and broadcast domination number for cactus, chordal, and $\delta$-hyperbolic graphs. Further, we prove that for all $r\geq 2$, \textsc{$r$-Multipacking} is \textsc{NP-complete} even for planar bipartite graphs with bounded degree, and also for bounded-diameter chordal and bounded-diameter bipartite graphs. For geometric variants, in $\mathbb{R}^2$ a maximum $1$-multipacking can be computed in polynomial time, but computing a maximum $2$-multipacking is \textsc{NP-hard}, and we provide approximation and parameterized algorithms for the $2$-multipacking problem.

==> Chapters/exchapter4_cactus.tex <==




\chapter{Multipacking on an unbounded hyperbolic graph-class: cactus graphs}\label{chapter:cactus}\hypertarget{chapter:introhref}{}
\minitoc 


% For a graph $G$, $ \MP(G) $ is the multipacking number, and $\gamma_b(G)$ is the broadcast domination number. It is known that $\MP(G)\leq \gamma_b(G)$ and  $\gamma_b(G)\leq 2\MP(G)+3$ for any graph $G$, and it was shown that $\gamma_b(G)-\MP(G)$ can be arbitrarily large for connected graphs. It is conjectured that  $\gamma_b(G)\leq 2\MP(G)$ for any general graph $G$. 


  In this chapter, we show that for any cactus  graph $G$,  $\gamma_b(G)\leq \frac{3}{2}\MP(G)+\frac{11}{2}$. Although cactus graphs form a narrow graph class, we used some non-trivial techniques to provide the bound. These techniques make an important step towards generating a tighter bound for general graphs. We also show that $\gamma_b(G)-\MP(G)$ can be arbitrarily large for cactus graphs and asteroidal triple-free graphs by constructing an infinite family of cactus graphs which are also asteroidal triple-free graphs such that the ratio $\gamma_b(G)/\MP(G)=4/3$, with $\MP(G)$ arbitrarily large.  Moreover, we provide an $O(n)$-time algorithm to construct a multipacking of cactus graph $G$ of size at least $ \frac{2}{3}\MP(G)-\frac{11}{3} $,  where $n$ is the number of vertices of the graph $G$. The hyperbolicity of the cactus graph class is unbounded. For $0$-hyperbolic graphs, $\MP(G)=\gamma_b(G)$. Moreover, $\MP(G)=\gamma_b(G)$ holds for the strongly chordal graphs which is a subclass of $\frac{1}{2}$-hyperbolic graphs. Now it's a natural question: what is the minimum value of $\delta$, for which we can say that the difference $ \gamma_{b}(G) -  \MP(G) $ can be arbitrarily large for $\delta$-hyperbolic graphs? We show that the minimum value of $\delta$ is $\frac{1}{2}$ using a construction of an infinite family of cactus graphs with hyperbolicity $\frac{1}{2}$.






\section{Chapter overview} 
In Section \ref{sec:Definitions and notation_cactus}, we recall some definitions and notations. In Section \ref{sec:inequality_linking_Broadcast domination_and_Multipacking}, we prove Theorem \ref{thm:multipacking_broadcast_relation}. In Section \ref{sec:approximation_algorithm_to_find_Multipacking}, we provide a $(\frac{3}{2}+o(1))$-factor approximation algorithm for finding multipacking on the cactus graphs. In Section \ref{sec:Unboundedness_of_the_gap_between_Broadcast_domination_and_Multipacking}, we prove  that the difference $ \gamma_{b}(G) -  \MP(G) $ can be arbitrarily large for cactus graphs. In Section \ref{sec:1/2-Hyperbolic graphs},  we show that the difference $ \gamma_{b}(G) -  \MP(G) $ can be arbitrarily large for $\frac{1}{2}$-hyperbolic graphs also.  We conclude this chapter in Section \ref{sec:conclusion_cactus}. 




\section{Preliminaries}\label{sec:Definitions and notation_cactus}


 Let $G=(V,E)$ be a graph and $d_G(u,v)$ be the length of a shortest path joining two vertices $u$ and $v$ in  $G$, we simply write $d(u,v)$ when there is no confusion. Let $diam(G)=\max\{d(u,v):u,v\in V(G)\}$. Diameter is a path of $G$  of the length  $diam(G)$. 
 $N_r[u]=\{v\in V:d(u,v)\leq r\}$ where $u\in V$. The \textit{eccentricity} $e(w)$  of a vertex $w$ is $\min \{r:N_r[w]=V\}$. The \textit{radius} of the graph $G$ is $\min\{e(w):w\in V\}$, denoted by $\rad(G)$.  The \textit{center set} $C(G)$ of the graph $G$  is the set of all vertices of minimum eccentricity, i.e., $C(G)=\{v\in V:e(v)=\rad(G)\}$. Each vertex in the set $C(G)$ is called a \textit{center} of the graph $G$.  
 A subgraph $H$ of a graph $G$ is called an \textit{isometric subgraph} if $d_H(u, v) = d_G(u, v)$ for every pair of vertices 
$u$ and $v$ in $H$, where $d_H(u,v)$ and $d_G(u,v)$ are the distances between $u$ and $v$ in $H$ and $G$, respectively. An \textit{isometric path} is an isometric subgraph which is a path.  If $H_1$ and $H_2$ are two subgraphs of $G$, then $H_1\cup H_2$ denotes the subgraph whose vertex set is $V(H_1)\cup V(H_2)$ and edge set is $E(H_1)\cup E(H_2)$. We denote an  indicator function as  $1_{[x<y]}$  that takes the value $1$ when $x<y$, and $0$ otherwise. If $P$ is a path in $G$, then we say $V(P)$ is the vertex set of the path $P$, $E(P)$ is the edge set of the path $P$, and  $l(P)$ is the length of the path $P$, i.e., $l(P)=|E(P)|$.

 A \textit{cactus} is a connected graph in which any two  cycles have at most one vertex in common. Equivalently, it is a connected graph in which every edge belongs to at most one  cycle.

  Let $d$ be the shortest-path metric of a graph $G$. The graph $G$ is called a \emph{$\delta$-hyperbolic graph} if for any four
vertices $u, v, w, x \in V(G)$, the two larger of the three sums $d(u, v) + d(w, x)$, $d(u, w) + d(v, x)$, $d(u, x) +
d(v, w)$ differ by at most $2\delta$. A graph class $\mathcal{G}$ is said to be hyperbolic if there exists a constant $\delta$ such that every graph $G \in \mathcal{G}$ is $\delta$-hyperbolic.






\section{Proof of Theorem \ref{thm:multipacking_broadcast_relation}}\label{sec:inequality_linking_Broadcast domination_and_Multipacking}


In this section, we prove a relation between the broadcast domination number and the radius of a cactus. Using this we establish our main result that relates the  broadcast domination number and the multipacking number for cactus graphs.




We start with a lemma that is true for general graphs. 


% Let $G$ be a graph with  a  center $c$  and $V_k=\{u\in V(G):d(c,u)=k\}$. So, $ V(G)=\bigcup_{k=0}^{r}V_k$. Let $P$ be a path in $G$, then we say $V(P)$ is the vertex set of the path $P$, $E(P)$ is the edge set of the path $P$, and  $l(P)$ is the length of the path $P$ i.e. $l(P)=|E(P)|$. Let $\rad(G)$ be the radius of $G$.

\begin{lemma} \label{lem:disjoint_radial_path} \textbf{(Disjoint radial path lemma)}
Let $G$ be a graph with radius $r$ and center $c$, where $r\geq 1$. Let $P$ be an isometric path in $G$ such that $l(P)=r$ and $c$ is one endpoint of $P$. Then there exists an isometric path $Q$ in $G$ such that $V(P)\cap V(Q)=\{c\}$, $ r-1 \leq l(Q)\leq  r$ and $c$ is one endpoint of $Q$.
\end{lemma}





% Let $G$ be a graph with $\rad(G)=r$ and center $c$. There exist two isometric paths $P$ and $Q$ in $G$ with the following properties:

% i) $P$ and $Q$ both have one end vertex $c$ and $V(P)\cap V(Q)=\{c\}$.           

% ii) $l(P)=r$ and $l(Q)=r-1$.



% $x\in  \bigcup\limits_{k=0}^{r-2}V_k$

The main idea of proving Lemma \ref{lem:disjoint_radial_path} is the following: if the length of all the isometric paths (except $P$) with one endpoint $c$  has length less than $r-1$, then the radius of $G$ will be less than $r$. In other case,  if all the isometric paths (except $P$) of length at least $r-1$ with one endpoint $c$     share at least one common vertex except $c$ with the path $P$, then also the radius of $G$ will be less than $r$. In both cases, we arrive at a contradiction.  The formal proof is the following.

\begin{proof}[Proof of Lemma \ref{lem:disjoint_radial_path}]


    Since $\rad(G)=r$, there exists a vertex $v_r$ such that $d(c,v_r)=r$. Let $P=(c,v_1,v_2,v_3,$ $\dots ,v_r)$ be an $r$ length path that joins $c$ and $v_r$. Therefore $P$ is an isometric path of $G$.  Let $Z_k$ be the set of all isometric paths of length $k$ whose one end vertex is $c$.  Since $d(c,v_{r-1})=r-1$, it implies $Z_{r-1}\neq \phi$. We prove this lemma using contradiction. We show that if  $(V(P)\cap V(Q))\setminus \{c\}\neq \phi$ for all $Q\in Z_{r-1}$, then $\rad(G)\leq r-1$.  
    
    Suppose  $(V(P)\cap V(Q))\setminus \{c\}\neq \phi$ for all $Q\in Z_{r-1}$.
    Let $V_k=\{u\in V(G):d(c,u)=k\}$. So, $ V(G)=\bigcup_{k=0}^{r}V_k$.  
     Let $w_r\in V_r$ and $P_1$ be a shortest path joining $c$ and $w_r$. Let $P_1=(c,w_1,w_2,w_3,\dots, w_r)$ and  $P_1'=(c,w_1,w_2,w_3,\dots, w_{r-1})$. So, $P_1'\in Z_{r-1}$. Therefore, $(V(P)\cap V(P_1'))\setminus \{c\}\neq \phi$. Let $w_t\in (V(P)\cap V(P_1'))\setminus \{c\}$ where $1\leq t \leq r-1$. Since $w_t,v_t\in V(P)\cap V_t$, so $w_t=v_t$. Now consider the path $P_1''=(v_1,v_2,\dots, v_t,w_{t+1},w_{t+2},\dots, w_r)$. Here $l(P_1'')=r-1$. Therefore $d(v_1,w_r)\leq r-1$. So, $d(v_1,w)\leq r-1$ for all $w\in V_r$. Let $u_{r-1}\in V_{r-1}$ and $P_2$ be a shortest path joining $c$ and $u_{r-1}$. Let $P_2=(c,u_1,u_2,u_3,\dots, u_{r-1})$. So, $P_2\in Z_{r-1}$. Therefore $(V(P)\cap V(P_2))\setminus \{c\}\neq \phi$. Let $u_s\in  (V(P)\cap V(P_2))\setminus \{c\}$ where $1\leq s\leq r-1$. Since $u_s,v_s\in V(P)\cap V_s$, so $u_s=v_s$. Now consider the path $P_2'=(v_1,v_2,\dots, v_s,u_{s+1},u_{s+2},\dots, u_{r-1})$. Here $l(P_2')=r-2$. Therefore $d(v_1,u_{r-1})\leq r-2$. So, $d(v_1,u)\leq r-2$ for all $u\in V_{r-1}$. Since $c$ and $v_1$ are adjacent, we can say that  $d(v_1,x)\leq r-1$ for all   $x\in  \bigcup_{k=0}^{r-2}V_k$. Therefore $d(v_1,x)\leq r-1$ for all $x\in V(G)$. This implies that $\rad(G)\leq r-1$. This is a contradiction. Therefore, there exists a path $Q\in Z_{r-1}$ such that $(V(P)\cap V(Q))\setminus \{c\}= \phi$.     
\end{proof}


For this section, we assume that $G$ is a cactus. 
Let $c$ be a center  and $r$ be the radius of $G$ where $r\geq 1$. We can find an isometric path $P$ of length $r$ whose one endpoint is $c$, since  $\rad(G)=r$. Let $P=(c,v_1,v_2,v_3,\dots ,v_r)$. Therefore, we can find an isometric path $Q$ in $G$ such that $V(P)\cap V(Q)=\{c\}$, $ r-1 \leq l(Q)\leq  r$ and $c$ is one endpoint of $Q$ by Lemma \ref{lem:disjoint_radial_path}. Let $Q=(c,w_1,w_2,w_3,\dots ,w_{r'})$ where $ r-1 \leq r'\leq  r$. Now we define some expressions to study the subgraph $P\cup Q$ in $G$ (See Fig. \ref{fig:bfs3}).  For $v_i\in V(P)\setminus \{c\}$ and $w_j\in V(Q)\setminus \{c\}$, we define  $ X_{P,Q}(v_i,w_j)=$\{$P_1$ :  $P_1$ is a path in $G$ that joins $v_i$ and $w_j$ such that $V(P)\cap V(P_1)=\{v_i\}$, $V(Q)\cap V(P_1)=\{w_j\}$ and $c \notin V(P_1)$\}. Let $X_{P,Q}=\{(v_i,w_j): X_{P,Q}(v_i,w_j)\neq \phi \}$. Since $G$ is a cactus, it implies every edge belongs to at most one cycle. Therefore, $|X_{P,Q}(v_i,w_j)|\leq 1$ and also $|X_{P,Q}|\leq 1$. Therefore, there is at most one path (say, $P_1$) that does not pass through $c$ and joins a vertex of $V(P)\setminus \{c\}$ with a vertex of $V(Q)\setminus \{c\}$ and $P_1$ intersects $P$ and $Q$ only at their joining points. So, the following observation is true. 

\begin{observation}
\label{obs:joining_path_atmost_1}
    Let $G$ be a cactus with $\rad(G)=r$ and center $c$. Suppose $P$ and $Q$  are two isometric paths  in $G$ such that   $V(P)\cap V(Q)=\{c\}$,  $l(P)=r$, $r-1\leq l(Q)\leq r$  and both have  one endpoint  $c$. Then 
    
    (i) $|X_{P,Q}|\leq 1$ and  $|X_{P,Q}(v_i,w_j)|\leq 1$ for all $(v_i,w_j)$.

(ii) $X_{P,Q}= \{(v_i,w_j)\}$ iff  $|X_{P,Q}(v_i,w_j)|= 1$.
    
\end{observation}




\begin{figure}[ht]
    \centering
    \includegraphics[scale = 0.8]{Figures/bfs3.pdf}
    \caption{The subgraph $P\cup Q\cup F_1\cup R'=H_\gamma (c_0,\alpha,c_t,\delta,c_m,\beta)$}
    \label{fig:bfs3}
\end{figure}







\medskip
\noindent \textbf{Finding a special subgraph $\bm{H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)}$  in cactus $\bm{G}$ : }
From Observation \ref{obs:joining_path_atmost_1}, there are two possible cases: either $|X_{P,Q}| =0$ or $|X_{P,Q}|=1$. First, we want to study the case when $|X_{P,Q}|=1$. In that case, suppose $ X_{P,Q}=\{(v_i,w_j)\}$ and $X_{P,Q}(v_i,w_j)=\{F_1\}$ (See Fig.  \ref{fig:bfs3}). We are interested in finding a multipacking set of $G$ from the subgraph $P\cup Q\cup F_1$.   Let $F_2=(v_i,v_{i-1},v_{i-2},\dots,v_1,c,w_1,w_2,\dots,$ $w_{j-1},w_j)$, $P'=(v_i,v_{i+1},\dots,v_{r})$ and $Q'=(w_j,w_{j+1},\dots,w_{r'})$. Here $F_1\cup F_2$ is a cycle and $P'$ and $Q'$ are two isometric paths that are attached to the cycle. Suppose there is another isometric path $R'$ which is disjoint with $P'$ and $Q'$ and whose one endpoint belongs to $V(F_2)$. Then  $P\cup Q\cup F_1\cup R'=F_1\cup F_2\cup P'\cup Q' \cup R'$ is a subgraph of $G$ (See Fig.\ref{fig:bfs3}).   Let $H=P\cup Q\cup F_1\cup R'$. Note that, we can always find $P$ and $Q$ in 
$G$ due to Lemma \ref{lem:disjoint_radial_path}, but  $F_1$ or $R'$ might not be there in $G$, in that case, we can assume that $V(F_1)$ or $V(R')$ is empty in $H$. In the rest of this section, our main goal is to find a multipacking of $G$ of size at least  $\frac{2}{3}\rad(G)-\frac{11}{3}$ from the subgraph $H$, so that we can prove Theorem \ref{thm:multipacking_broadcast_relation}. To give $H$ a general structure, we want to rename the vertices. Suppose  $F_1\cup F_2$ is a cycle of length $\gamma$. Let $F_1\cup F_2=C_\gamma=(c_0,c_1,c_2,\dots,c_{\gamma-2},c_{\gamma-1},c_0)$. Suppose $l(P')=\alpha$, $l(Q')=\beta$ and $l(R')=\delta$. We rename the paths $P'$, $Q'$ and $R'$ as $P_{\alpha+1}$, $Q_{\beta+1}$ and $R_{\delta+1}$ respectively. 
Let $P_{\alpha+1}=(a_0,a_{1},\dots,a_{\alpha})$,  $Q_{\beta+1}=(b_0,b_{1},\dots,b_{\beta})$ and  $R_{\delta+1}=(e_0,e_{1},\dots,e_{\delta})$   such that $c_0=a_0$,  $c_t=e_0$, $c_m=b_0$  (See Fig. \ref{fig:bfs1}). Here $P_{\alpha+1}$, $Q_{\beta+1}$ and $R_{\delta+1}$ are three isometric paths in $G$.  According to the structure, we have $V(P_{\alpha+1})\cap V(Q_{\beta+1})=\phi$,  $V(Q_{\beta+1}) \cap V(R_{\delta+1}) =\phi$,
$V(R_{\delta+1})\cap V(P_{\alpha+1})=\phi$,
$V(C_\gamma)\cap V(P_{\alpha+1}) =\{c_0\}$, $V(C_\gamma)\cap V(R_{\delta+1})=\{c_t\}$, $V(C_\gamma)\cap V(Q_{\beta+1})=\{c_m\}$. Now we can write $H$ as a variable of $\alpha, \beta, \gamma $ and $\delta$. Let $H=H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)$. 



\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{Figures/bfs1.pdf}
    \caption{The subgraph $H_\gamma (c_0,\alpha,c_t,\delta,c_m,\beta)$}
    \label{fig:bfs1}
\end{figure}



In the rest of the section, we study how to find a multipacking of $G$ from the subgraph $H_\gamma(c_0,\alpha,c_t,$ $\delta,c_m,\beta)$. Using this, we prove Lemma \ref{lem:multipacking_radius_relation} that yields Theorem \ref{thm:multipacking_broadcast_relation} which is our main result in this section. 












\begin{lemma} [\cite{beaudou2019broadcast}]  \label{lem:isometric_path}
    Let $G$ be a graph, $k$ be a positive integer and $P=(v_0,v_1, \dots ,$ $ v_{k-1})$ be an isometric path in $G$ with $k$ vertices. Let $M = \{v_i:0\leq i\leq k, i\equiv 0 \text{ (mod $3$)} \}$ be the set of every third vertex
on this path. Then $M$ is a multipacking in $G$ of size $\big\lceil\frac{k}{3}\big\rceil$.
\end{lemma}


Note that, if $H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)$ is a subgraph of $G$, then $P_{\alpha+1}$, $Q_{\beta+1}$ and $R_{\delta+1}$ are three isometric paths in $G$ by the definition of $H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)$. Moreover, since $G$ is a cactus, two cycles cannot share an edge. Therefore, the following observation is true.


\begin{observation} 
\label{obs:isometric_graph}
    If $G$ is a cactus and $H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)$ is a subgraph of $G$ such that $\gamma\geq 3 $ and $c_0,c_t,c_m$ are distinct vertices of $C_\gamma$, then $H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)$ is an isometric subgraph of $G$.
\end{observation}    








\begin{observation} 
\label{obs:isometric_graph_path_F_1}
    Let $G$ be a cactus and $H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)$ be a subgraph of $G$ such that $\gamma\geq 3 $ and $c_0,c_t,c_m$ are distinct vertices of $C_\gamma$. Let $F_1$ and $F_2$ be two paths such that  $F_1=(c_m,c_{m+1},\dots,$ $c_{\gamma-1},c_0)$ and $F_2=(c_0,c_1,\dots,c_m)$. Then
    
 \noindent  (i)  If $l(F_1)> l(F_2)$, then $P_{\alpha+1}\cup F_2\cup Q_{\beta +1}$ is an isometric path of $G$.    


 \noindent (ii)  If $l(F_1)<l(F_2)$, then $P_{\alpha+1}\cup F_1\cup Q_{\beta +1}$ is an isometric path of $G$. 

 \noindent (iii) If $l(F_1)=l(F_2)$, then 
 both of $P_{\alpha+1}\cup F_1\cup Q_{\beta +1}$ and $P_{\alpha+1}\cup F_2\cup Q_{\beta +1}$ are isometric paths of $G$. 

   
\end{observation}    






The following lemma tells why it is sufficient to find multipacking in $H_\gamma(c_0,\alpha,$ $c_t,\delta,c_m,\beta)$ to provide a multipacking in $G$. 









\begin{lemma}   
\label{lem:multipacking_subgraph}
    Let $G$ be a cactus and $H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)$ be a subgraph of $G$. If   $M$ is a multipacking of $H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)$, then $M$ is a  
 multipacking of $G$.
\end{lemma}



\begin{proof} 
Let $H=H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)$. Since $M$ is multipacking of $H$, therefore $|N_r[z]\cap M|\leq r$ for all $z\in V(H)$ and $r\geq 1$. Let $z\in V(G)\setminus V(H)$ and    $v\in V(H)$.  Define $ P_H(z,v)=$\{$P$ :  $P$ is a path in $G$ that joins $z$ and $v$ such that $V(P)\cap V(H)=\{v\}$\}. 
% and $P(z,H)=\bigcup_{v\in H} P_H(z,v)$.
Note that, if $v_1,v_2\in V(H)$ and $v_1\neq v_2$, then $P_H(z,v_1)\cap P_H(z,v_2)=\phi$. Since $G$ is connected, therefore $|\{v\in V(H):P_H(z,v)\neq \phi\}|\geq 1$.
 

\medskip
\noindent
\textbf{Claim \ref{lem:multipacking_subgraph}.1. }  If $z\in V(G)\setminus V(H)$, then $|\{v\in V(H):P_H(z,v)\neq \phi\}|\leq 2$. 
% If $z\in V(G)\setminus V(H)$, then  


\begin{claimproof}Suppose $|\{v\in V(H):P_H(z,v)\neq \phi\}|\geq 3$. Let $v_1,v_2,v_3\in \{v\in V(H):P_H(z,v)\neq \phi\}$ where $v_1,v_2,v_3$ are distinct. So, there are $3$ distinct paths $P_1,P_2,P_3$ such that $P_i\in P_H(z,v_i)$ for $i=1,2,3$. Then there are two cycles formed by the paths $P_1,P_2,P_3$ that have at least one common edge, which is a contradiction, since $G$ is a cactus.     
\end{claimproof}

\vspace{0.2cm}
\noindent
\textbf{Claim \ref{lem:multipacking_subgraph}.2. }    If $z\in V(G)\setminus V(H)$ and  $|\{v\in V(H):P_H(z,v)\neq \phi\}|=1 $, then  $|N_r[z]\cap M|\leq r$ for all $r\geq 1$.


\begin{claimproof} Let $ \{v\in V(H):P_H(z,v)\neq \phi\}=\{v_1\}$. Therefore,  if $v$ is any vertex in $V(H)$, then  any path joining $z$ and $v$ passes through $v_1$. Let $d(z,v_1)=k$ for some $k\geq 1$. We have $|N_{r}[v_1]\cap M|\leq r$ for all $r\geq 1$. If $1\leq r<k$, then  $|N_r[z]\cap M|=0<r$. If $r\geq k$, then $|N_r[z]\cap M|= |N_{r-k}[v_1]\cap M|\leq r-k\leq r$.   
\end{claimproof}

\vspace{0.2cm}
\noindent
\textbf{Claim \ref{lem:multipacking_subgraph}.3. }    If $z\in V(G)\setminus V(H)$ and $|\{v\in V(H):P_H(z,v)\neq \phi\}|=2 $, then  $|N_r[z]\cap M|\leq r$ for all $r\geq 1$.


\begin{claimproof} Let $\{v\in V(H):P_H(z,v)\neq \phi\}=\{v_1,v_2\}$. Therefore,  if $w$ is any vertex in $V(H)$, then  any path joining $z$ and $w$ passes through $v_1$ or $v_2$. Note that, both of  $v_1,v_2$ belongs to either $P_{\alpha+1}$, $Q_{\beta+1}$ or $R_{\delta+1}$, otherwise $G$ cannot be a cactus. W.l.o.g. assume that $v_1,v_2\in P_{\alpha+1}$.  Let $d(z,v_1)=k_1$ and $d(z,v_2)=k_2$ for some $k_1,k_2\geq 1$. Since $P_{\alpha+1}$ is an isometric path in $G$, therefore $d(v_1,v_2)\leq d(z,v_1)+d(z,v_2)=k_1 + k_2$. Let $r$ be a positive integer  and  $S=V(H)$. If $N_{r-k_1}[v_1]\cap N_{r-k_2}[v_2]\cap S=\phi$,  then  $(r-k_1)+(r-k_2)\leq d(v_1,v_2)\leq k_1+k_2$ $\implies$ $r\leq k_1+k_2$. Therefore,   $|N_r[z]\cap M|=|N_{r-k_1}[v_1]\cap M|+|N_{r-k_2}[v_2]\cap M|\leq r-k_1+r-k_2=2r-(k_1+k_2)\leq r$. Suppose  $N_{r-k_1}[v_1]\cap N_{r-k_2}[v_2]\cap S\neq \phi$. Let $v_1=a_i$, $v_2=a_j$, $h=\big\lfloor\frac{i+j}{2}\big\rfloor$, $v=a_h$ and $s=\big\lfloor\frac{(r-k_1)+(r-k_2)+ d(v_1,v_2)+1}{2}\big\rfloor$.  So, $N_r[z]\cap S=(N_{r-k_1}[v_1]\cup N_{r-k_2}[v_2])\cap S\subseteq N_s[v]\cap S$ $\implies$ $N_r[z]\cap M\subseteq N_s[v]\cap M$ $\implies$ $|N_r[z]\cap M|\leq |N_s[v]\cap M|\leq s= \big\lfloor\frac{(r-k_1)+(r-k_2)+ d(v_1,v_2)+1}{2}\big\rfloor\leq \big\lfloor\frac{(r-k_1)+(r-k_2)+ k_1+k_2+1}{2}\big\rfloor\leq \big\lfloor\frac{2r+1}{2}\big\rfloor= \big\lfloor r+\frac{1}{2}\big\rfloor= r$.   
\end{claimproof} 


From the above results, we can say that   $|N_{r}[z]\cap M|\leq r$ for all $z\in V(G)$ and $r\geq 1$. Therefore, $M$ is a   multipacking of $G$. 
% then $|N_r[z]\cap M|=\big\lfloor\frac{(r-k_1)+(r-k_2)+ d(v_1,v_2)+1}{3}\big\rfloor\leq \big\lfloor\frac{(r-k_1)+(r-k_2)+ k_1+k_2+1}{3}\big\rfloor\leq \big\lfloor\frac{2r+1}{3}\big\rfloor\leq r$. \hfill $\square$ \hfill $\square$
\end{proof}







Now our goal is to find multipacking of $H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)$. Whatever multipacking we find for the subgraph $H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)$, that will be a multipacking for $G$ by Lemma \ref{lem:multipacking_subgraph}. There could be several ways to choose a multipacking set from the subgraph $H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)$. 
% [But we have to ensure that the size of the multipacking is at least $\frac{2}{3}\rad(G)-\frac{11}{3}$ for proving the Lemma \ref{lem:multipacking_radius_relation} which is the main lemma to prove Theorem \ref{thm:multipacking_broadcast_relation}].  
But in order to prove the Lemma \ref{lem:multipacking_radius_relation} which is the main lemma to prove Theorem \ref{thm:multipacking_broadcast_relation}, we have to ensure that the size of the multipacking is at least $\frac{2}{3}\rad(G)-\frac{11}{3}$.

We discuss three choices to find  a  multipacking in $H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)$ in the following subsections.

From now,  we can write $H$ in place of $H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)$ for the simplicity. 


% htp
\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{Figures/m_2.pdf}
 \caption{ The circles and squares  represent the  subgraph $P_{\alpha+1}\cup \overline{P}_{\alpha_1+1}\cup Q_{\beta+1}\cup \overline{Q}_{\beta_1+1}$ and the squares represent the set $M_\gamma(c_0,\alpha,\alpha_{1},c_m,\beta,\beta_1)$ in this figure.}
    \label{fig:m_2}
\end{figure}

\medskip
\noindent\textbf{Finding a multipacking of  $\bm{H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)} $ 
 according to Choice-1 :}\label{subec:multipacking_technique_1}
\smallskip





Here we find two paths of  $H$ so that the set of every third vertex (with some exceptions) 
on those paths provide a multipacking of $H$. Let $\overline{P}_{\alpha_1+1}=(c_0,c_1,\dots,c_{\alpha_1})$
and $\overline{Q}_{\beta_1+1}=(c_m,c_{m+1},\dots,c_{m+\beta_1})$ where $0\leq \alpha_1\leq m-1$ and $0\leq \beta_1\leq (\gamma-1)-m$. Now we choose every third vertex (with some exceptions) from the paths  $P_{\alpha+1}\cup \overline{P}_{\alpha_1+1}$ and $Q_{\beta+1}\cup \overline{Q}_{\beta_1+1}$ to construct a set, called $M_\gamma(c_0,\alpha,\alpha_1,c_m,\beta,\beta_1)$ (See Fig. \ref{fig:m_2}). Formally we can define,  $M_\gamma(c_0,\alpha,\alpha_1,c_m,\beta,\beta_1)=\{a_i:0\leq i\leq \alpha,i\equiv 0 \text{ (mod $3$)}\}\cup \{c_i:0\leq i\leq \alpha_1, i\equiv 0 \text{ (mod $3$)}\}\cup \{b_i:0\leq i\leq \beta, i\equiv 0 \text{ (mod $3$)}\}\cup \{c_i:m\leq i\leq m+\beta_1, i\equiv m \text{ (mod $3$)}\}\setminus\{c_0,c_m\}$.  This set will be a multipacking of $G$ under the conditions stated in the following lemma.







\begin{lemma} 
\label{lem:multipacking_subgraph1}
Let $G$ be a cactus and $H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)$  be a subgraph of $G$. Let  $\alpha_1,\alpha_2,\beta_1,\beta_2$ be non negative integers such that $\alpha_2=(m-1)-\alpha_1 $, $\beta_2=(\gamma-1)-(m+\beta_1) $. If $\alpha_1\leq 3\beta_2+\alpha_2+\beta_1$ and $\beta_1\leq 3\alpha_2+\beta_2+\alpha_1$, then 
 $M_\gamma(c_0,\alpha,\alpha_1,c_m,\beta,\beta_1)$  is a multipacking of $G$ of size at least
 $ \big\lfloor\frac{\alpha+\alpha_1+1}{3}\big\rfloor+\big\lfloor\frac{\beta+\beta_1+1}{3}\big\rfloor -2$. 


   
\end{lemma}



\begin{proof}

Let $H=H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)$,  $M=M_\gamma(c_0,\alpha,\alpha_1,c_m,\beta,\beta_1)$.


Let $v=c_{x_1}$ for some $x_1$ where $0\leq x_1\leq m-1$. Note that, $m-1=\alpha_1+\alpha_2$ and $\gamma=\alpha_1+\alpha_2+\beta_1+\beta_2+2$  or $\big\lfloor\frac{\gamma}{2}\big\rfloor=\big\lfloor\frac{\beta_{1}+\beta_{2}+\alpha_{1}+\alpha_2}{2}\big\rfloor+1$.





Recall that, we denote an  indicator function as  $1_{[x<y]}$  that takes the value $1$ when $x<y$, and $0$ otherwise.
























\vspace{0.22cm}

 \noindent \textit{\textbf{Case 1: }} $1\leq r\leq \max\{\alpha_{1}+\alpha_2-x_1,\beta_{2}+x_1\}$. 

 $|N_r(v)\cap M|\leq \frac{1}{3} [\{2r-2(\alpha_{1}+\alpha_2-x_1)-1+(\alpha_1-x_1)+r+1\}\times 1_{[\alpha_{1}+\alpha_2-x_1\leq \beta_{2}+x_1]}+\{r-x_1-\beta_{2}+2r+1\}\times 1_{[\alpha_{1}+\alpha_2-x_1> \beta_{2}+x_1]}]\leq r $. Therefore $|N_r(v)\cap M|\leq r$.

\vspace{0.22cm}


 \noindent \textit{\textbf{Case 2: }} $\max\{\alpha_{1}+\alpha_2-x_1,\beta_{2}+x_1\}<r\leq \big\lfloor\frac{\beta_{1}+\beta_{2}+\alpha_{1}+\alpha_2}{2}\big\rfloor$. 

 $|N_r(v)\cap M|\leq \frac{1}{3} [ r+1+(\alpha_1-x_1)+2\{r-(\alpha_{1}+\alpha_2-x_1)\}-1+r-(x_1+\beta_{2})]=\frac{1}{3} [4r-\alpha_{1}-\beta_{2}-2\alpha_2]$.
We know that $\beta_{1}\leq \alpha_{1}+\beta_{2}+3\alpha_2$ $\implies$ $\beta_{1}+\beta_{2}+\alpha_{1}+\alpha_2\leq 2\alpha_{1}+2\beta_{2}+4\alpha_2$ $\implies$ $\frac{\beta_{1}+\beta_{2}+\alpha_{1}+\alpha_2}{2}\leq \alpha_{1}+\beta_{2}+2\alpha_2$. Since $r\leq \big\lfloor\frac{\beta_{1}+\beta_{2}+\alpha_{1}+\alpha_2}{2}\big\rfloor$, therefore $r\leq \alpha_{1}+\beta_{2}+2\alpha_2$  $\implies$ $4r-\alpha_{1}-\beta_{2}-2\alpha_2\leq 3r$ $\implies$ $|N_r(v)\cap M|\leq r$. 


\vspace{0.22cm}




 \noindent \textit{\textbf{Case 3: }} $\big\lfloor\frac{\beta_{1}+\beta_{2}+\alpha_{1}+\alpha_2}{2}\big\rfloor< r$. 
 
 $|N_r(v)\cap M|\leq \frac{1}{3} [\beta_{1}+1+\alpha_{1}+1+(r-x_1)+r-(\alpha_{1}+\alpha_2-x_1+1)]=\frac{1}{3} [2r+\beta_{1}-\alpha_2+1]$. We know that $\beta_{1}\leq \alpha_{1}+\beta_{2}+3\alpha_2$ $\implies$ $2\beta_{1}-2\alpha_2\leq \beta_{1}+\beta_{2}+\alpha_{1}+\alpha_2$ $\implies$ $\beta_{1}-\alpha_2\leq \frac{\beta_{1}+\beta_{2}+\alpha_{1}+\alpha_2}{2}$  $\implies$ $\beta_{1}-\alpha_2+1\leq \frac{\beta_{1}+\beta_{2}+\alpha_{1}+\alpha_2}{2}+1$ $\implies$ $\beta_{1}-\alpha_2+1\leq \big\lfloor\frac{\beta_{1}+\beta_{2}+\alpha_{1}+\alpha_2}{2}\big\rfloor+1\leq r$ 
 $\implies$ $\beta_{1}-\alpha_2 +1\leq r$ $\implies$ $|N_r(v)\cap M|\leq \frac{1}{3} [2r+\beta_{1}-\alpha_2+1]\leq r$.


\vspace{0.22cm}




% \begin{figure}
%     \centering
%     \includegraphics[  height=5.5cm]{m(2)1.pdf}
%  \caption{$S_\gamma(c_0,\alpha,\alpha_1,c_m,\beta,\beta_1)$}
%     \label{fig:m(2)1}
% \end{figure}




 Similarly, using the relation $\alpha_1\leq 3\beta_2+\alpha_2+\beta_1$, we can show that, when $v=c_{x_2}$ for some $x_2$ where $m\leq x_2\leq \gamma-1$, we can show that  $v\in \{c_i:m\leq i\leq \gamma-1\}$, then $|N_r(v)\cap M|\leq r$ for all  $r\geq 1$. Therefore, $|N_r(v)\cap M|\leq r$ for all $v\in V(C_\gamma)$ and $r\geq 1$.

 Suppose $v\in V(P_{\alpha+1})$, then any path that joins $v$ with a vertex in $V(C_\gamma)\cup V(Q_{\beta+1})\cup V(R_{\delta+1})$ passes through $a_0$, otherwise $G$ cannot be a cactus. By Observation \ref{obs:isometric_graph} we know that $H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)$ is an isometric subgraph of $G$.  Therefore $|N_r(v)\cap M|\leq r$ for all  $r\geq 1$. Similarly we can show that, if $v$ is in  $V(Q_{\beta+1})$ or $V(R_{\delta+1})$, then $|N_r(v)\cap M|\leq r$ for all  $r\geq 1$. Therefore $M$ is a multipacking of $H$. So, $M$ is a multipacking of $G$ by Lemma \ref{lem:multipacking_subgraph} and $|M|\geq  \big\lfloor\frac{\alpha+\alpha_1+1}{3}\big\rfloor+\big\lfloor\frac{\beta+\beta_1+1}{3}\big\rfloor -2$.   
\end{proof}  





Substitute $\alpha_2=(m-1)-\alpha_1 $ and $\beta_2=(\gamma-1)-(m+\beta_1) $ in Lemma \ref{lem:multipacking_subgraph1}. This yields the following.




 

\begin{lemma} 
\label{lem:gamma/2}
    Let $G$ be a cactus and $H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)$  be a subgraph of $G$. Let  $\alpha_1$ and $\beta_1$ be non negative integers such that $\alpha_1\leq m-1$ and $\beta_1\leq (\gamma-1)-m$. If $\alpha_1\leq \big\lfloor\frac{\gamma}{2}\big\rfloor-1$ and $\beta_1\leq \big\lfloor\frac{\gamma}{2}\big\rfloor-1$, then 
 $M_\gamma(c_0,\alpha,\alpha_1,c_m,\beta,\beta_1)$  is a multipacking of $G$ of size at least
 $ \big\lfloor\frac{\alpha+\alpha_1+1}{3}\big\rfloor+\big\lfloor\frac{\beta+\beta_1+1}{3}\big\rfloor -2$.
 
\end{lemma}

% \begin{proof}

%  Let  $\alpha_2=(m-1)-\alpha_1 $ and $\beta_2=(\gamma-1)-(m+\beta_1) $.  Therefore, $\gamma=\alpha_1+\alpha_2+\beta_1+\beta_2+2$. Here $\alpha_1\leq \big\lfloor\frac{\gamma}{2}\big\rfloor-1$ $\implies$  $\alpha_1\leq \frac{\gamma}{2}-1$  $\implies$  $\alpha_1\leq \frac{\alpha_1+\alpha_2+\beta_1+\beta_2+2}{2}-1$  $\implies$ $\alpha_1\leq \alpha_2+\beta_1+\beta_2$ $\implies$ $\alpha_1\leq \alpha_2+\beta_1+3\beta_2$. Similarly, $\beta_1\leq \big\lfloor\frac{\gamma}{2}\big\rfloor-1$ $\implies$ $\beta_1\leq \alpha_1+3\alpha_2+\beta_2$. Therefore, $M_\gamma(c_0,\alpha,\alpha_1,c_m,\beta,\beta_1)$  is a multipacking of $G$ of size at least
% $ \big\lfloor\frac{\alpha+\alpha_1+1}{3}\big\rfloor+\big\lfloor\frac{\beta+\beta_1+1}{3}\big\rfloor -2$ by Lemma \ref{lem:multipacking_subgraph1}. \hfill $\square$
% \end{proof}






\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{Figures/multipacking_choice_2.pdf}
 \caption{The circles and squares  represent the subgraph $P_{\alpha+1}\cup C_\gamma$  and the squares represent the  set $M'_\gamma(c_0,\alpha)$ in this figure.}
    \label{fig:multipacking_choice_2}
\end{figure}

\smallskip
\noindent \textbf{Finding a multipacking of  $\bm{H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)} $ according to Choice-2 :}\label{subec:multipacking_technique_2}
\medskip










Here we find a path and a cycle of  $H$ so that the set of every third vertex (with some exceptions) 
on these subgraphs provide a multipacking of $H$. Consider the path $P_{\alpha+1}$ and the cycle $C_\gamma$. Now we choose every third vertex (with some exceptions) from these subgraphs  to construct a set, called $M'_\gamma(c_0,\alpha)$ (See Fig. \ref{fig:multipacking_choice_2}).  Formally we can define,  $M'_\gamma(c_0,\alpha)=\{a_i:0\leq i\leq \alpha, i\equiv 0 \text{ (mod $3$)}\}\cup \{c_i:0\leq i\leq \gamma-1,i\equiv 0 \text{ (mod $3$)}\}\setminus \{c_0\}$. 

Similarly, for  the path $Q_{\beta+1}$ and the cycle $C_\gamma$, we define the set $M'_\gamma(c_m,\beta)=\{b_i:0\leq i\leq \beta, i\equiv 0 \text{ (mod $3$)}\}\cup \{c_i:0\leq i\leq \gamma-1,i\equiv m \text{ (mod $3$)}\}\setminus \{c_m\}$. 
These sets will be a multipacking of $G$ under the conditions stated in the following lemma.



\begin{lemma} 
\label{lem:multipacking_delta=0}
     Let $G$ be a cactus and $H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)$  be a subgraph of $G$. Then $M'_\gamma(c_0,\alpha)$ is a multipacking of $G$ of size at least $\big\lfloor\frac{\gamma}{3}\big\rfloor+\big\lfloor\frac{\alpha}{3}\big\rfloor-1$ and $M'_\gamma(c_m,\beta)$ is a multipacking of $G$ of size at least $\big\lfloor\frac{\gamma}{3}\big\rfloor+\big\lfloor\frac{\beta}{3}\big\rfloor-1$.
\end{lemma}



\begin{proof}  Let $H=H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)$,  $M'=M'_\gamma(c_0,\alpha)$.  From the definition of $M'$,   $|N_r(v)\cap M'|\leq r$ for all $v\in V(H)$ and $r\geq 1$. Hence $M'$ is a multipacking of $H$ size at least 
  $\big\lfloor\frac{\gamma}{3}\big\rfloor+\big\lfloor\frac{\alpha}{3}\big\rfloor-1$. Therefore, $M'$ is a multipacking of $G$ by Lemma \ref{lem:multipacking_subgraph}. By the similar reason $M'_\gamma(c_m,\beta)$ is a multipacking of $G$ of size at least $\big\lfloor\frac{\gamma}{3}\big\rfloor+\big\lfloor\frac{\beta}{3}\big\rfloor-1$. 
\end{proof}


\begin{figure}[htp]
    \centering
    \includegraphics[width=\textwidth]{Figures/m2_11.pdf}
 \caption{The circles and squares  represent the subgraph $P_{\alpha+1}\cup \overline{R}_{\delta,\delta_1}\cup C_\gamma$   and the squares represent the  set $M'_\gamma(c_0,\alpha,c_t,\delta,\delta_1)$ in this figure.}
    \label{fig:m2_11}
\end{figure}

\medskip
\medskip
\medskip
\medskip
\medskip
\medskip
\medskip
\medskip
\medskip
\medskip
\medskip
\medskip
\noindent\textbf{Finding a multipacking in  $\bm{H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)} $ according to Choice-3 :}\label{subec:multipacking_technique_3}
\smallskip





Next, we discuss a more general choice, similar to the last one. In the last choice, we did not use the path $R_{\delta+1}$ to construct a multipacking. Here we are going to use $R_{\delta+1}$ also when it is there in $G$. Let   $\overline{R}_{\delta,\delta_1}=(e_{\delta_1+1},e_{\delta_1+2},\dots,e_{\delta})$ which is a path and a part of the path $R_{\delta+1}$. 
Now we choose every third vertex (with some exceptions) from the subgraphs $P_{\alpha+1}$, $\overline{R}_{\delta,\delta_1}$ and $C_\gamma$   to construct a set, called $M'_\gamma(c_0,\alpha,c_t,\delta,\delta_1)$(See Fig. \ref{fig:m2_11}). Formally we can define,  $M'_\gamma(c_0,\alpha,c_t,\delta,\delta_1)=\{a_i:0\leq i\leq \alpha, i\equiv 0 \text{ (mod $3$)}\}\cup \{e_i:\delta_1+2\leq i\leq \delta,i\equiv \delta_1+1 \text{ (mod $3$)}\}\cup \{c_i:0\leq i\leq \gamma-1,i\equiv 0 \text{ (mod $3$)}\}\setminus \{c_0\}$.




Similarly, if we consider the subgraphs $Q_{\beta+1}$, $\overline{R}_{\delta,\delta_1}$ and $C_\gamma$, we can define,  $M'_\gamma(c_m,\beta,$ $ c_t,\delta,\delta_1)=\{b_i:0\leq i\leq \beta, i\equiv 0 \text{ (mod $3$)}\}\cup \{e_i:\delta_1+2\leq i\leq \delta,i\equiv \delta_1+1 \text{ (mod $3$)}\}\cup \{c_i:0\leq i\leq \gamma-1,i\equiv m \text{ (mod $3$)}\}\setminus \{c_m\}$.


These sets will be a multipacking of $G$ under some conditions, that has been stated in the following lemma.

\begin{lemma}  
\label{lem:delta1}
     Let $G$ be a cactus and $H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)$  be a subgraph of $G$.  If $\delta_1=\big\lfloor\frac{\gamma}{2}\big\rfloor-d(c_0,c_t)$ and  $ \delta\geq \delta_1$, then $M'_\gamma(c_0,\alpha,c_t,\delta,\delta_1)$ is a multipacking of $G$ of size at least $\big\lfloor\frac{\gamma}{3}\big\rfloor+\big\lfloor\frac{\alpha}{3}\big\rfloor+ \big\lfloor\frac{\delta-\delta_1}{3}\big\rfloor-1$. Moreover, if $\delta_2=\big\lfloor\frac{\gamma}{2}\big\rfloor-d(c_m,c_t)$ and $ \delta\geq \delta_2$, then $M'_\gamma(c_m,\beta,c_t,\delta,\delta_2)$ is a multipacking of $G$ of size at least $\big\lfloor\frac{\gamma}{3}\big\rfloor+\big\lfloor\frac{\beta}{3}\big\rfloor+ \big\lfloor\frac{\delta-\delta_2}{3}\big\rfloor-1$.
\end{lemma}



\begin{proof} Let $H=H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)$,  $M'=M'_\gamma(c_0,\alpha,c_t,\delta,\delta_1)$.


Here $V(C_\gamma)=\{c_i:0\leq i\leq \gamma-1\}$. 
Let $v=c_{x_1}$ for some $x_1$ where $0\leq x_1\leq \gamma-1$. Let  $d_1=d(c_0,v)$ and $d_2=d(c_t,v)$. Since $c_0,c_t\in V(C_\gamma)$,  $d(c_0,c_t)\leq diam(C_\gamma)= \big\lfloor\frac{\gamma}{2}\big\rfloor$. Therefore $\big\lfloor\frac{\gamma}{2}\big\rfloor- d(c_0,c_t)\geq 0\implies \delta_1\geq 0$. 

\vspace{0.22cm}

 \noindent \textit{\textbf{Case 1: }}
    $1\leq r \leq \max\{d_1,d_2+\delta_1\}$.

In that case, $|N_r(v)\cap M'|\leq r$ for $v\in V(C_\gamma)$.
    
  
\vspace{0.22cm}
   
 \noindent \textit{\textbf{Case 2: }}  $ \max\{d_1,d_2+\delta_1\}<r$. 
 
 $|N_r(v)\cap M'|\leq \frac{1}{3}[r+1+r-d_1+r-\delta_1]=\frac{1}{3}[3r+1-d_1-\delta_1]\leq r$.

 \vspace{0.22cm}

 Suppose $v\in V(P_{\alpha+1})$, then any path that joins $v$ with a vertex in $V(C_\gamma)\cup V(Q_{\beta+1})\cup V(R_{\delta+1})$ passes through $a_0$, otherwise $G$ cannot be a cactus. By Observation \ref{obs:isometric_graph} we know that $H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)$ is an isometric subgraph of $G$.  Therefore $|N_r(v)\cap M'|\leq r$ for all  $r\geq 1$. Similarly we can show that, if $v\in V(Q_{\beta+1})$ or $v \in V(R_{\delta+1})$, then $|N_r(v)\cap M'|\leq r$ for all  $r\geq 1$. Therefore $M'$ is a multipacking of $H$. So, $M'$ is a multipacking of $G$ by Lemma \ref{lem:multipacking_subgraph}. $M'_\gamma(c_0,\alpha,c_t,\delta,\delta_1)$ is a multipacking of $G$ of size at least $\big\lfloor\frac{\gamma}{3}\big\rfloor+\big\lfloor\frac{\alpha}{3}\big\rfloor+ \big\lfloor\frac{\delta-\delta_1}{3}\big\rfloor-1$.
 
 Similarly, we can show that, if $\delta_2=\big\lfloor\frac{\gamma}{2}\big\rfloor-d(c_m,c_t)$ and $ \delta\geq \delta_2$, then $M'_\gamma(c_m,\beta,c_t,$ $\delta,\delta_2)$ is a multipacking of $G$ of size at least $\big\lfloor\frac{\gamma}{3}\big\rfloor+\big\lfloor\frac{\beta}{3}\big\rfloor+ \big\lfloor\frac{\delta-\delta_2}{3}\big\rfloor-1$.  
\end{proof}





Now we are ready to prove Lemma  \ref{lem:multipacking_radius_relation}. Here is a small observation before we start proving the lemma. We use this observation in the proof.

\begin{observation}
\label{obs:r/3} If $r$ is a positive integer, then 
    $\big\lfloor\frac{r}{3}\big\rfloor+\big\lfloor\frac{r-1}{3}\big\rfloor \geq \big\lfloor\frac{2r-1}{3}\big\rfloor-1$,   $\big\lfloor\frac{r}{3}\big\rfloor\geq \frac{r}{3}-\frac{2}{3}$,  and $\big\lfloor\frac{r}{2}\big\rfloor+\big\lceil\frac{r}{2}\big\rceil=r$.


    % $\frac{r}{3}+\frac{2}{3}\geq \big\lceil\frac{r}{3}\big\rceil$,

    % $\big\lfloor\frac{r}{2}\big\rfloor\geq \frac{r}{2}-\frac{1}{2}$

    % If $r$ and $k$ are two positive integers, then $\big\lfloor\frac{r}{k}\big\rfloor\geq \frac{r}{k}-\frac{k-1}{k}$.
\end{observation}







\begin{lemma} 
    \label{lem:multipacking_radius_relation}
  Let $G$ be a cactus with radius $\rad(G)$, then  $\MP(G)\geq \frac{2}{3}\rad(G)-\frac{11}{3}$.
\end{lemma}

\begin{proofsketch}     First, we present a very brief sketch of the proof for Lemma \ref{lem:multipacking_radius_relation}. Let $\rad(G)=r$ and $c$ be a center of $G$. If $r=0$ or $1$, then $\MP(G)=1$. Therefore, for $r\leq 1$, we have $\MP(G)\geq \frac{2}{3}\rad(G)$. Now assume $r\geq 2$. Since $G$ has radius $r$, there is an isometric path $P$ in $G$ whose one endpoint  is $c$ and $l(P)=r$. Let $Q$ be a  largest isometric path in $G$ whose one endpoint  is $c$ and  $V(P)\cap V(Q)=\{c\}$. If $l(Q)=r'$, then $ r-1 \leq r'\leq  r$  by Lemma \ref{lem:disjoint_radial_path}.
    Let $P=(v_0,v_1, \dots , v_{r})$ and  $Q=(w_0,w_1, \dots , w_{r'})$ where $v_0=w_0=c$. From Observation \ref{obs:joining_path_atmost_1}, we know that $|X_{P,Q}|\leq 1$. 

     If  $|X_{P,Q}|=0$, we take the path $P\cup Q$ which is an isometric path of length $r+r'$ and choose every third vertex to the path to construct a multipacking of size at least $\MP(G)\geq \big\lceil\frac{2}{3}\rad(G)\big\rceil$ by Lemma \ref{lem:isometric_path}.

     Suppose $|X_{P,Q}|=1$. We have already discussed in this section that we can find a subgraph $H_\gamma(c_0,\alpha,c_t,\delta,$ $c_m,\beta)$ in $G$ and we use Lemma \ref{lem:gamma/2}, Lemma \ref{lem:multipacking_delta=0} and Lemma \ref{lem:delta1} under several cases to construct a multipacking of size at least $ \frac{2}{3}\rad(G)-\frac{11}{3}$.   
\end{proofsketch}




\begin{proof}[Proof of Lemma \ref{lem:multipacking_radius_relation}] Let $\rad(G)=r$ and $c$ be a center of $G$. If $r=0$ or $1$, then $\MP(G)=1$. Therefore, for $r\leq 1$, we have $\MP(G)\geq \frac{2}{3}\rad(G)$. Now assume $r\geq 2$. Since $G$ has radius $r$, there is an isometric path $P$ in $G$ whose one endpoint  is $c$ and $l(P)=r$. Let $Q$ be a  largest isometric path in $G$ whose one endpoint  is $c$ and  $V(P)\cap V(Q)=\{c\}$. If $l(Q)=r'$, then $ r-1 \leq r'\leq  r$  by Lemma \ref{lem:disjoint_radial_path}.
    Let $P=(v_0,v_1, \dots , v_{r})$ and  $Q=(w_0,w_1, \dots , w_{r'})$ where $v_0=w_0=c$. From Observation \ref{obs:joining_path_atmost_1}, we know that $|X_{P,Q}|\leq 1$.   

\vspace{0.2cm}
\noindent
\textbf{Claim \ref{lem:multipacking_radius_relation}.1. } If  $|X_{P,Q}|=0$, then $\MP(G)\geq \big\lceil\frac{2}{3}\rad(G)\big\rceil$.

\begin{claimproof} Since  $|X_{P,Q}|=0$,  any path in $G$ that joins a vertex of $P$ with a vertex of $Q$ always passes through $c$. Therefore, $P\cup Q$ is an isometric path of length $r+r'$ and $|V(P\cup Q)|=r+r'+1$. By Lemma \ref{lem:isometric_path}, there is a multipacking in $G$ of size $\big\lceil\frac{r+r'+1}{3}\big\rceil$. Since $r'\geq r-1$, $\big\lceil\frac{r+r'+1}{3}\big\rceil \geq \big\lceil\frac{2r}{3}\big\rceil$.  Therefore, $\MP(G)\geq \big\lceil\frac{2r}{3}\big\rceil$.    
\end{claimproof} 

\medskip

Suppose $|X_{P,Q}|=1$. Let $X_{P,Q}=\{(v_i,w_j)\}$. Then $|X_{P,Q}(v_i,w_j)|=1$ by Observation \ref{obs:joining_path_atmost_1}. Let  $F_1\in X_{P,Q}(v_i,w_j)$ and $F_2=(v_i,v_{i-1},v_{i-2},\dots,v_1,v_0,$ $w_1,w_2,\dots,$ $w_{j-1},w_j)$. Therefore, $F_1$ and $F_2$ form a cycle $F_1\cup F_2$ of length  $ l(F_1)+l(F_2)$. Note that $l(F_1)\geq 1$, since $v_i\neq w_j$. Let $\gamma= l(F_1)+l(F_2)$ and  $C_\gamma=(c_0,c_1,c_2,\dots,c_{\gamma-2},$ $c_{\gamma-1},c_0) $ be a cycle of length $\gamma$.  Therefore,  $C_\gamma$ is  isomorphic to $ F_1\cup F_2$. For simplicity, we assume that $C_\gamma = F_1\cup F_2$. So, we can  assume that  $F_2=(c_0,c_1,c_2,\dots,$ $c_{m})$ and $F_1=(c_m,c_{m+1},\dots,c_{\gamma-1}, c_0)$.  
 Since $P$ and $Q$ are isometric paths, therefore $P'=(v_i,v_{i+1},\dots,v_{r})$ and $Q'=(w_j,w_{j+1},\dots,w_{r'})$ are also isometric paths in $G$.  Therefore $C_\gamma\cup P'\cup Q'$ can be represented as 
 $H_\gamma(c_0,\alpha,c_t,0,c_m,\beta)$ or $ H_\gamma(c_0,\alpha,c_m,\beta)$, where $\alpha =l(P')$ and $\beta=l(Q')$. So, $C_\gamma\cup P'\cup Q'$ is an isometric subgraph of $G$ by Observation \ref{obs:isometric_graph}. Let $H=C_\gamma\cup P'\cup Q'$. For simplicity, we can assume that $P'=P_{\alpha+1}=(a_0,a_1,\dots,a_{\alpha+1})$ and $Q'=Q_{\beta+1}=(b_0,b_1,\dots,b_{\alpha+1})$. (See. Fig. \ref{fig:bfs3} and Fig. \ref{fig:bfs1}) 
 
 \vspace{0.2cm}
\noindent
\textbf{Claim \ref{lem:multipacking_radius_relation}.2. }  If  $|X_{P,Q}|=1$ and $l(F_1)\geq  l(F_2)$, then $\MP(G)\geq \big\lceil\frac{2}{3}\rad(G)\big\rceil$.

\begin{claimproof}
Since $G$ is a cactus and $l(F_1)\geq  l(F_2)$,  
$P\cup Q$ is an isometric path in $G$ by Observation \ref{obs:isometric_graph_path_F_1}.  Note that  $l(P\cup Q)=r+r'$ and $|V(P\cup Q)|=r+r'+1$. By Lemma \ref{lem:isometric_path}, we can say that, there is a multipacking in $G$ of size $\big\lceil\frac{r+r'+1}{3}\big\rceil$. Now $r'\geq r-1$ $\implies$ $\big\lceil\frac{r+r'+1}{3}\big\rceil \geq \big\lceil\frac{2r}{3}\big\rceil$.  Therefore, $\MP(G)\geq \big\lceil\frac{2r}{3}\big\rceil$.  
\end{claimproof}
 
 
 
 \medskip
 
 Now assume $l(F_1)<  l(F_2)$. Therefore $F_1\cup P'\cup Q'$ is an isometric path by Observation \ref{obs:isometric_graph_path_F_1}. We know $l(F_2)=m$. Let $l(F_1)=x$   and $g=m+\big\lfloor\frac{x}{2}\big\rfloor$. Therefore $c_g$ is a middle point of the path $F_1$. Let $S_r=\{u\in V(G):d(c_g,u)=r\}$.  Here  $S_r\neq \phi$, since $\rad(G)=r$. We know that $c$ is a center of $G$ and  $c \in V(C_\gamma)$, more precisely $c\in V(F_2)$. Therefore $c=c_k$ for some $k\in \{0,1,2,\dots,m\}$. Let $F_2^1=(c_0,c_1,\dots,c_k)$ and $F_2^2=(c_k,c_{k+1},\dots,c_m)$. Therefore $F_2=F_2^1\cup F_2^2$. Let  $l(F_2^1)=y$ and $l(F_2^2)=z$. Therefore, $F_1\cup F_2^1\cup F_2^2=C_\gamma$ and $x+y+z=\gamma$. Note that  $d(c_g,c_m)=d_H(c_g,c_m)=\big\lfloor\frac{x}{2}\big\rfloor$ and $d(c_g,c_0)=d_H(c_g,c_0)=x-\big\lfloor\frac{x}{2}\big\rfloor=\big\lceil\frac{x}{2}\big\rceil$.  We know that $l(P')=\alpha $ and $l(Q')=\beta$. Therefore $\alpha +y=l(P')+l(F^1_2)=l(P)=r$ and $\beta+z=l(Q')+l(F^2_2)=l(Q)=r'$. From now we use all these notations in the upcoming results.


Now we want to show that,  if   $l(F_1)<  l(F_2)$, then $x$, $y$ and $z$ are upper bounded by $\big\lfloor\frac{\gamma}{2}\big\rfloor$.  
 $l(F_1)<  l(F_2)\implies x<y+z\implies x<\frac{x+y+z}{2}\implies x<\frac{\gamma}{2} \implies x\leq \big\lfloor\frac{\gamma}{2}\big\rfloor$.  Since $P$ is an isometric path, $F_2^1$ is a shortest path joining $c_0$ and $c$. Note that, the path  $ F_2^2\cup F_1$  also  joins $c_0$ and $c$. Therefore, $l(F_2^1)\leq l(F_2^2\cup F_1)\implies l(F_2^1)\leq l(F_2^2)+l(F_1)\implies y\leq z+x \implies y\leq \frac{x+y+z}{2}\implies y\leq \big\lfloor\frac{\gamma}{2}\big\rfloor$. Similarly, we can show that  $z\leq \big\lfloor\frac{\gamma}{2}\big\rfloor$, since $F_2^2$ is a shortest path joining $c_0$ and $c$. 
 Therefore, if $l(F_1)<  l(F_2)$ , $\max\{x,y,z\}\leq \big\lfloor\frac{\gamma}{2}\big\rfloor$. 

\vspace{0.2cm}
\noindent
\textbf{Claim \ref{lem:multipacking_radius_relation}.3. }  If  $|X_{P,Q}|=1$, $l(F_1)<  l(F_2)$ and $S_r\cap P'\neq \phi $, then $\MP(G)\geq \big\lfloor\frac{2}{3}\rad(G)-\frac{1}{3}\big\rfloor-3$.

\begin{claimproof}
   Let $u\in S_r\cap P'$. Let $\alpha_1=x-1$ and  $\beta_1=z-1$.  Since $F_1\cup P' \cup Q' $ is an isometric path of $G$,   $\alpha+\alpha_1+1=x+\alpha =  d(c_m,v_r)\geq d(c_g,u)=r $. Here $\beta+\beta_1+1=z+\beta=r'\geq r-1$. We have $\alpha_1=x-1\leq \big\lfloor\frac{\gamma}{2}\big\rfloor-1$ and $\beta_1=z-1\leq \big\lfloor\frac{\gamma}{2}\big\rfloor-1$, since $\max\{x,y,z\}\leq \big\lfloor\frac{\gamma}{2}\big\rfloor$. We have shown that $H$ can be represented as 
 $ H_\gamma(c_0,\alpha,c_t,0,c_m,\beta) $. Therefore, there is a multipacking of $G$ of size at least 
  $ \big\lfloor\frac{\alpha+\alpha_1+1}{3}\big\rfloor+\big\lfloor\frac{\beta+\beta_1+1}{3}\big\rfloor -2$ by Lemma \ref{lem:gamma/2}.  
 Here $  \big\lfloor\frac{\alpha+\alpha_1+1}{3}\big\rfloor+\big\lfloor\frac{\beta+\beta_1+1}{3}\big\rfloor -2\geq \big\lfloor\frac{r}{3}\big\rfloor+\big\lfloor\frac{r-1}{3}\big\rfloor -2\geq \big\lfloor\frac{2r-1}{3}\big\rfloor-3$ by Observation \ref{obs:r/3}. 
\end{claimproof}







\vspace{0.2cm}
\noindent
\textbf{Claim \ref{lem:multipacking_radius_relation}.4. }  If  $|X_{P,Q}|=1$, $l(F_1)<  l(F_2)$ and $S_r\cap Q'\neq \phi $, then $\MP(G)\geq 2\big\lfloor\frac{\rad(G)}{3}\big\rfloor-2$.

\begin{claimproof}
Let $u\in S_r\cap Q'$. Let $\alpha_1=y-1$ and   $\beta_1=x-1$.  Since $F_1\cup P' \cup Q' $ is an isometric path of $G$, $\beta+\beta_1+1=x+\beta=d(c_0,w_{r'})\geq d(c_g,u)=r $. Moreover, $\alpha+\alpha_1+1=y+\alpha =  r$.  We have $\alpha_1=y-1\leq \big\lfloor\frac{\gamma}{2}\big\rfloor-1$ and $\beta_1=x-1\leq \big\lfloor\frac{\gamma}{2}\big\rfloor-1$, since $\max\{x,y,z\}\leq \big\lfloor\frac{\gamma}{2}\big\rfloor$. We have shown that $H$ can be represented as 
 $ H_\gamma(c_0,\alpha,c_t,0,c_m,\beta) $. Therefore,  there is a multipacking of $G$ of size at least 
  $ \big\lfloor\frac{\alpha+\alpha_1+1}{3}\big\rfloor+\big\lfloor\frac{\beta+\beta_1+1}{3}\big\rfloor -2$ by Lemma \ref{lem:gamma/2}. 
 Here $  \big\lfloor\frac{\alpha+\alpha_1+1}{3}\big\rfloor+\big\lfloor\frac{\beta+\beta_1+1}{3}\big\rfloor -2\geq \big\lfloor\frac{r}{3}\big\rfloor+\big\lfloor\frac{r}{3}\big\rfloor -2\geq 2\big\lfloor\frac{r}{3}\big\rfloor-2$.  
\end{claimproof}








\vspace{0.2cm}
\noindent
\textbf{Claim \ref{lem:multipacking_radius_relation}.5. } If  $|X_{P,Q}|=1$, $l(F_1)<  l(F_2)$ and $S_r\cap C_\gamma \neq \phi $, then $\MP(G)\geq \big\lceil\frac{2}{3}\rad(G)\big\rceil$.

\begin{claimproof}
    We know that $ H_\gamma(c_0,0,c_t,0,c_m,0)= C_\gamma$.  Therefore $C_\gamma$ is an isometric subgraph of $G$ by Observation \ref{obs:isometric_graph}. $S_r\cap C_\gamma \neq \phi \implies r\leq \big\lceil\frac{\gamma}{2}\big\rceil\implies 2r\leq \gamma$. Let $M=\{c_i:0\leq i\leq \gamma-1,i\equiv 0 \text{ (mod $3$)}\}$. Note that, $M$ is a multipacking of $C_\gamma$. Therefore, $M$ is a mutipacking of $G$ by Lemma \ref{lem:multipacking_subgraph}.  Here $|M|=\big\lceil\frac{\gamma}{3}\big\rceil\geq \big\lceil\frac{2r}{3}\big\rceil$, since $2r\leq \gamma$.   
\end{claimproof}















\vspace{0.2cm}
\noindent
\textbf{Claim \ref{lem:multipacking_radius_relation}.6. } If  $|X_{P,Q}|=1$, $l(F_1)<  l(F_2)$ and $S_r\cap V(H) =\phi $, then $\MP(G)\geq \frac{2}{3}\rad(G)-\frac{11}{3}$.


\begin{claimproof} Let $u\in S_r$. Therefore, $u\notin V(H)$. We know that $g=m+\big\lfloor\frac{x}{2}\big\rfloor$. Let $R$ be a shortest path joining $c_g$ and $u$. Therefore, $R$ is an isometric path of $G$. Let $R=(u_0,u_1,\dots,u_r)$ where $c_g=u_0$ and $u=u_r$. Suppose $h=\max\{i:u_i\in V(H)\}$.   Let $R'=(u_{h+1},u_{h+2},\dots,u_r)$. 

First, we show that  $u_h\notin V(F_1)$. Suppose $u_h\in V(F_1)$, so $u_h\in \{c_m,c_{m+1},\dots,$ $c_{\gamma-1},c_0\}$. Therefore, $u_h=c_{g'}$ for some $g'\in \{m,m+1,\dots,\gamma-1,0\}$. First consider $u_h\in \{c_{g+1},c_{g+2},\dots,$ $c_{\gamma-1},c_0\}$. We know that $c$ is a center of $G$ and $c=c_k$ for some $k\in \{0,1,2,\dots,m\}$. Suppose $(c_k,c_{k-1},\dots,c_0,c_{\gamma-1},\dots,c_{g'})$ is a shortest path joining $c_k(=c)$ and $c_{g'}(=u_h)$.  We have shown that $H$ is an isometric subgraph of $G$. Therefore, the distance between two vertices in $H$ is the distance in $G$.
Since $S_r\cap V(H)= \phi$, we have $d(c_g,v_r)<r$. Therefore,  $d(c_g,v_r)<r=d(c_g,u)\implies d(c_g,v_r)<d(c_g,u) \implies d(c_g,u_h)+d(u_h,c_0)+d(c_0,v_r)<d(c_g,u_h)+d(u_h,u)\implies d(u_h,c_0)+d(c_0,v_r)<d(u_h,u)\implies d(c_0,v_r)<d(u_h,u)$.   Since $c$ is a center of $G$ and $S_r\cap V(H)= \phi$, we have $r\geq d(c,u)=d(c,c_0)+d(c_0,u_h)+d(u_h,u)>d(c,c_0)+d(c_0,u_h)+d(c_0,v_r)=d(c,v_r)+d(c_0,u_h)=r+d(c_0,u_h)\implies d(c_0,u_h)<0$. This is a contradiction. Now assume $(c_k,c_{k+1},\dots,c_m,c_{m+1},\dots,c_{g'})$ is a shortest path joining $c$ and $u_h$. Since $c$ is a center of $G$ and $S_r\cap V(H)= \phi$, we have $r\geq d(c,u)=d(c,c_g)+d(c_g,u)=d(c,c_g)+r\implies d(c,c_g)=0\implies c=c_g$. Therefore $r=d(c,v_{r})=d(c_g,v_r)\implies v_r\in S_r\cap V(H)$, which is a contradiction. 
Therefore, $u_h\notin \{c_{g+1},c_{g+2},\dots,c_{\gamma-1},c_0\}$. Similarly we can show that $u_h\notin \{c_{m},c_{m+1},\dots,c_{g-1},c_g\}$. So, $u_h\notin V(F_1)$.


If $u_h\in V(P')$, then $d(c_g,u)=r>d(c_g,v_r)\implies d(c_g,u_h)+d(u,u_h)>d(c_g,u_h)+d(u_h,v_r)\implies d(u,u_h)>d(u_h,v_r)\implies d(u,u_h)+d(c,u_h)>d(u_h,v_r)+d(c,u_h)\implies d(c,u)>d(c,v_r)\implies d(c,u)>r$, which is a contradiction, since $c$ is a center of the graph $G$ having radius $r$. Therefore, $u_h\notin V(P')$. Similarly, we can show that $u_h\notin V(Q')$.

% If $u_h$ belongs to $ V(P')$ or $V(Q')$, then $d(c,u)>r$. This is a contradiction, since $c$ is center of $G$ having radius $r$. Therefore, $u_h\notin V(P')\cup V(Q')$.

% First, we show that  $u_h\notin V(F_1)$. Suppose $u_h\in V(F_1)$, $s=h$. Since  $T$ is an isometric path of $G$, $d(c_g,u_s)=s$. We have $s\leq \max\{d_H(c_g,c_0),d_H(c_g,c_m)\}\leq  \big\lceil\frac{x}{2}\big\rceil$, since $u_s\in V(F_1)$. Now,  $S_r\cap V(H) =\phi \implies d(c_g,v_r)<r \implies d_H(c_g,v_r)<r \implies d_H(c_g,c_0)+d_H(c_0,v_r)<r \implies \big\lceil\frac{x}{2}\big\rceil+r-y<r \implies \big\lceil\frac{x}{2}\big\rceil<y \implies s<y$. Therefore, $y-s>0$ and $\big\lceil\frac{x}{2}\big\rceil-s\geq 0$.  Here, the path $T'=(u_s,u_{s+1},\dots, u_r)$ is an isometric path in $G$, since $T$ is an isometric path in $G$. Therefore, $C_\gamma\cup P'\cup Q'\cup T'\cong H_\gamma(c_0,\alpha,c_t,\delta,c_m,\beta)$ where $\alpha =l(P'), \beta =l(Q')$ and $\delta=l(T')$. By Observation \ref{obs:isometric_graph}, $C_\gamma\cup P'\cup Q'\cup T'$ is an isometric subgraph of $G$. Now, we calculate the distance between the center $C$ and $u$. $\dots$ $u_h\notin V( P'\cup Q')$. 



Therefore $u_h\in V(C_\gamma)\setminus V(F_1)= \{c_1,c_2,\dots,c_{m-1}\}$.  Since $G$ is a cactus, therefore every edge belongs to almost one cycle. This implies that $u_i\in V(C_\gamma)$ for all $0\leq i\leq h$.  Let $u_h=c_t$. 

Suppose $x\geq \alpha $, then $x+y+z+\beta\geq \alpha +y+z+\beta\geq r+r'\geq 2r-1$.  By Lemma \ref{lem:multipacking_delta=0},  $M'_\gamma(c_m,\beta)$ is a multipacking of $G$ of size at least $\big\lfloor\frac{\gamma}{3}\big\rfloor+\big\lfloor\frac{\beta}{3}\big\rfloor-1$. Therefore  $\big\lfloor\frac{\gamma}{3}\big\rfloor+\big\lfloor\frac{\beta}{3}\big\rfloor-1\geq \frac{\gamma}{3}-\frac{2}{3}+\frac{\beta}{3}-\frac{2}{3}-1=\frac{x+y+z+\beta}{3}-\frac{7}{3}\geq \frac{2r-1}{3}-\frac{7}{3}$. 

Suppose $x\geq \beta$, then $x+y+z+\alpha \geq \alpha +y+z+\beta\geq r+r'\geq 2r-1$.  By Lemma \ref{lem:multipacking_delta=0},  $M'_\gamma(c_0,\alpha )$ is a multipacking of $G$ of size at least $\big\lfloor\frac{\gamma}{3}\big\rfloor+\big\lfloor\frac{\alpha }{3}\big\rfloor-1$ (See Fig. \ref{fig:multipacking_choice_2}). Therefore  $\big\lfloor\frac{\gamma}{3}\big\rfloor+\big\lfloor\frac{\alpha }{3}\big\rfloor-1\geq \frac{\gamma}{3}-\frac{2}{3}+\frac{\alpha }{3}-\frac{2}{3}-1=\frac{x+y+z+\beta}{3}-\frac{7}{3}\geq \frac{2r-1}{3}-\frac{7}{3}$. 

Now assume $x<\min\{\alpha ,\beta\}$.

Note that, $S_r\cap V(H)=\phi\implies S_r\cap V(C_\gamma)=\phi$. Therefore, there is no vertex on the cycle $C_\gamma$ which is at  distance $r$ from the vertex $c_g$. Therefore, $r>\big\lfloor\frac{\gamma}{2}\big\rfloor$.

Now we split the remainder of the proof  into two cases. 


    
\vspace{0.22cm} 

 \noindent \textit{\textbf{Case 1: }} $ \big\lfloor\frac{\gamma}{2}\big\rfloor<r\leq \big\lfloor\frac{\gamma}{2}\big\rfloor+\big\lfloor\frac{x}{2}\big\rfloor$.

 Consider the set $M'_\gamma(c_0,\alpha )$. This a multipacking of $G$ of size $\big\lfloor\frac{\gamma}{3}\big\rfloor+\big\lfloor\frac{\alpha }{3}\big\rfloor-1$ by Lemma \ref{lem:multipacking_delta=0}. Now $\big\lfloor\frac{\gamma}{3}\big\rfloor+\big\lfloor\frac{\alpha }{3}\big\rfloor-1\geq
 \big\lfloor\frac{\gamma}{3}\big\rfloor+\big\lfloor\frac{x}{3}\big\rfloor-1\geq
 \frac{\gamma}{3}-\frac{2}{3}+\frac{x}{3}-\frac{2}{3}-1\geq \frac{2}{3}.\big(\frac{\gamma}{2}+\frac{x}{2}\big)-\frac{7}{3}\geq \frac{2}{3}r-\frac{7}{3}$.




\vspace{0.22cm} 

 \noindent \textit{\textbf{Case 2: }} $ \big\lfloor\frac{\gamma}{2}\big\rfloor+\big\lfloor\frac{x}{2}\big\rfloor<r$.


Now consider  
 $\delta=r-d(c_g,c_t)$, $\delta_1=\big\lfloor\frac{\gamma}{2}\big\rfloor-d(c_0,c_t)$ and $\delta_2=\big\lfloor\frac{\gamma}{2}\big\rfloor-d(c_m,c_t)$.  Since $c_0,c_t\in V(C_\gamma)$,  $d(c_0,c_t)\leq diam(C_\gamma)= \big\lfloor\frac{\gamma}{2}\big\rfloor$. Therefore $\big\lfloor\frac{\gamma}{2}\big\rfloor- d(c_0,c_t)\geq 0\implies \delta_1\geq 0$. Similarly, we can show that $\delta_2\geq 0$. Now $\delta-\delta_1=r-d(c_g,c_t)-\big\lfloor\frac{\gamma}{2}\big\rfloor+d(c_0,c_t)\geq r-d(c_g,c_0)-d(c_0,c_t)-\big\lfloor\frac{\gamma}{2}\big\rfloor+d(c_0,c_t)\geq r-\big\lceil\frac{x}{2}\big\rceil-\big\lfloor\frac{\gamma}{2}\big\rfloor\geq 0$. Therefore $\delta \geq \delta_1$ and $\delta - \delta_1\geq r-\big\lceil\frac{x}{2}\big\rceil-\big\lfloor\frac{\gamma}{2}\big\rfloor\geq 0$. Similarly, we can show that $\delta\geq \delta_2$ and $\delta - \delta_2\geq r-\big\lceil\frac{x}{2}\big\rceil-\big\lfloor\frac{\gamma}{2}\big\rfloor\geq 0$.  Now we are ready to use Lemma \ref{lem:delta1} to find multipacking in $G$. 


% Let $t_1=\min\{t,s\}$. Therefore, $2t_1\leq t+s \leq t+s+x=y+z+x=\gamma\implies t_1\leq \frac{\gamma}{2}\implies t_1\leq \big\lfloor\frac{\gamma}{2}\big\rfloor$. We have $ \big\lfloor\frac{\gamma}{2}\big\rfloor+\big\lfloor\frac{x}{2}\big\rfloor<r\implies  \big\lfloor\frac{\gamma}{2}\big\rfloor+\big\lceil\frac{x}{2}\big\rceil\leq r \implies  t_1+\big\lceil\frac{x}{2}\big\rceil\leq r $. Note that, $l(T')=r-\min\{\big\lceil\frac{x}{2}\big\rceil+t,\big\lfloor\frac{x}{2}\big\rfloor+s\}\geq r-\min\{\big\lceil\frac{x}{2}\big\rceil+t,\big\lceil\frac{x}{2}\big\rceil+s\} \geq  r-\big\lceil\frac{x}{2}\big\rceil-t_1$. Let 
% $\delta_1=\big\lfloor\frac{\gamma}{2}\big\rfloor-t_1$ and $\delta=r-\big\lceil\frac{x}{2}\big\rceil-t_1$. Note that, $\delta\geq 0$ and $\delta_1\geq 0$. 

First assume that, $z\geq y$. 
By Lemma \ref{lem:delta1},   $M'_\gamma(c_0,\alpha ,c_t,\delta,\delta_1)$ is a multipacking of $G$ of size at least $\big\lfloor\frac{\gamma}{3}\big\rfloor+\big\lfloor\frac{\alpha }{3}\big\rfloor+ \big\lfloor\frac{\delta-\delta_1}{3}\big\rfloor-1$.  Now, $\big\lfloor\frac{\gamma}{3}\big\rfloor+\big\lfloor\frac{\alpha }{3}\big\rfloor+ \big\lfloor\frac{\delta-\delta_1}{3}\big\rfloor-1\geq
\frac{\gamma}{3}-\frac{2}{3}+\frac{\alpha }{3}-\frac{2}{3}+\frac{\delta-\delta_1}{3}-\frac{2}{3}-1=
\frac{\gamma}{3}+\frac{\alpha }{3}+\frac{1}{3}.\big(r-\big\lceil\frac{x}{2}\big\rceil-\big\lfloor\frac{\gamma}{2}\big\rfloor\big)-3   
\geq  \frac{\gamma}{3}+\frac{\alpha }{3}+\frac{1}{3}.\big(r-\frac{x}{2}-1-\frac{\gamma}{2}\big)-3 =
\frac{1}{3}\big(r+\frac{\gamma}{2}-\frac{x}{2}+\alpha \big) -\frac{10}{3}\geq 
\frac{1}{3}\big(r+\frac{\gamma}{2}-\frac{x}{2}+r-y\big) -\frac{10}{3}\geq
\frac{1}{3}\big(2r+\frac{x+y+z}{2}-\frac{x}{2}-y\big) -\frac{10}{3}\geq
\frac{1}{3}\big(2r+\frac{z-y}{2}\big) -\frac{10}{3}\geq \frac{2}{3}r-\frac{10}{3}$.




Suppose $z<y$. By Lemma \ref{lem:delta1},   $M'_\gamma(c_m,\beta,c_t,\delta,\delta_2)$ is a multipacking of $G$ of size at least $\big\lfloor\frac{\gamma}{3}\big\rfloor+\big\lfloor\frac{\beta}{3}\big\rfloor+ \big\lfloor\frac{\delta-\delta_2}{3}\big\rfloor-1$.  Now, $\big\lfloor\frac{\gamma}{3}\big\rfloor+\big\lfloor\frac{\beta}{3}\big\rfloor+ \big\lfloor\frac{\delta-\delta_2}{3}\big\rfloor-1\geq
\frac{\gamma}{3}-\frac{2}{3}+\frac{\beta}{3}-\frac{2}{3}+\frac{\delta-\delta_2}{3}-\frac{2}{3}-1=
\frac{\gamma}{3}+\frac{\beta}{3}+\frac{1}{3}.\big(r-\big\lceil\frac{x}{2}\big\rceil-\big\lfloor\frac{\gamma}{2}\big\rfloor\big)-3   
\geq  \frac{\gamma}{3}+\frac{\beta}{3}+\frac{1}{3}.\big(r-\frac{x}{2}-1-\frac{\gamma}{2}\big)-3 =
\frac{1}{3}\big(r+\frac{\gamma}{2}-\frac{x}{2}+\beta\big) -\frac{10}{3}\geq 
\frac{1}{3}\big(r+\frac{\gamma}{2}-\frac{x}{2}+r'-z\big) -\frac{10}{3}\geq
\frac{1}{3}\big(r+r-1+\frac{x+y+z}{2}-\frac{x}{2}-z\big) -\frac{10}{3}\geq
\frac{1}{3}\big(2r+\frac{y-z}{2}\big) -\frac{11}{3}\geq \frac{2}{3}r-\frac{11}{3}$. 
\end{claimproof}


In each case, $G$ has a multipacking of size at least $ \frac{2}{3}\rad(G)-\frac{11}{3}$. Therefore, $\MP(G)\geq \frac{2}{3}\rad(G)-\frac{11}{3}$.  
\end{proof}





\begin{theorem}[\cite{teshima2012broadcasts,erwin2001cost}]  \label{thm:mpGleqgammabG}  If $G$ is a connected graph of order at least 2  having radius $ \rad(G) $, multipacking number  $\MP(G) $, broadcast domination number $ \gamma_{b}(G) $ and domination number $\gamma(G)$, then $ \MP(G)\leq \gamma_{b}(G) \leq min\{\gamma (G),\rad(G)\}$.
\end{theorem} 




\begin{proof}[Proof of Theorem \ref{thm:multipacking_broadcast_relation}]
    We have $\gamma_b(G)\leq \rad(G)$ from Theorem \ref{thm:mpGleqgammabG}. From Lemma 
\ref{lem:multipacking_radius_relation}, we get $\MP(G)\geq \frac{2}{3}\rad(G)-\frac{11}{3}$ . Therefore, $ \frac{2}{3}.\gamma_b(G)-\frac{11}{3}\leq \MP(G)\implies \gamma_b(G)\leq \frac{3}{2}\MP(G)+\frac{11}{2}$.
\end{proof}






\section{An approximation algorithm to find multipacking in cactus graphs}\label{sec:approximation_algorithm_to_find_Multipacking}

We provide the following algorithm to approximate multipacking of a cactus graph. This algorithm is a direct implementation of the proof of Theorem \ref{thm:multipacking_broadcast_relation}.

\smallskip
\noindent\textbf{Approximation algorithm: } Since $G$ is a cactus graph,  we can find a center $c$ and  an isometric path $P$ of length $r$ whose one endpoint is $c$ in $O(n)$-time, where $n$ is the number of vertices of $G$. After that, we can find another isometric path $Q$ having length $r-1$ or $r$ whose one endpoint is $c$ and $V(P)\cap V(Q)=\{c\}$.  Then the flow of the proof of 
Lemma  \ref{lem:multipacking_radius_relation} provides an $O(n)$-time algorithm to construct a multipacking of size at least $\frac{2}{3}\rad(G)-\frac{11}{3}$. Thus we can find  a multipacking of $G$ of size at least $\frac{2}{3}\rad(G)-\frac{11}{3}$ in $O(n)$-time.  Moreover,  $\MP(G)\geq \frac{2}{3}\rad(G)-\frac{11}{3}\geq \frac{2}{3}\MP(G)-\frac{11}{3}$ by Theorem \ref{thm:mpGleqgammabG}. This implies the existence of a $(\frac{3}{2}+o(1))$-factor approximation algorithm for
the multipacking problem on cactus graph. Therefore, we have the following.

\MultipackingAlgorithm*




\section{Unboundedness of the gap between broadcast domination and multipacking number of cactus and AT-free graphs}\label{sec:Unboundedness_of_the_gap_between_Broadcast_domination_and_Multipacking}



In this section, we prove that the difference between the broadcast domination number and the multipacking number of the cactus and AT-free graphs can be arbitrarily large.  
 Moreover, we make a connection with the \emph{fractional} versions of the two concepts dominating broadcast and multipacking for cactus and AT-free graphs.















To prove that the difference $ \gamma_{b}(G) -  \MP(G) $ can be arbitrarily large, we construct the graph $G_k$ as follows. Let $A_i=(a_i,b_i,c_i,d_i,e_i,a_i)$ be a 5-cycle  for each  $i=1,2,\dots,3k$. We form $G_k $ by joining $b_i$ to $e_{i+1}$ for each $i=1,2,\dots,3k-1$ (See Fig. \ref{fig:pentagon}). This  graph is a  cactus graph (and AT-free graph). We show that $\MP(G_k)=3k$ and $\gamma_b(G_k)=4k$. 



\begin{figure}[ht]
    \centering

\includegraphics[width=\textwidth]{Figures/pentagon.pdf}
    \caption{The $G_k$ graph with $\gamma_b(G_k)=4k$ and $\MP(G_k)=3k$. The set $\{a_i:1\leq i\leq 3k\}$ is a maximum multipacking of $G_k$.} 
    \label{fig:pentagon}
\end{figure}




\begin{lemma} \label{lem:mpGk=3k} $\MP(G_{k})=3k$, for each positive integer $k$.
\end{lemma}

\begin{proof} The path $P=(e_1,a_1,b_1,e_2,a_2,b_2,\dots,e_{3k}a_{3k}b_{3k})$ is a diametral path of $G_k$ (Fig.\ref{fig:pentagon}). This implies $P$ is an isometric path of $G_k$ having the length  $l(P)=3.3k-1$. By Lemma \ref{lem:isometric_path}, every third vertex on this path form a multipacking of size $\big\lceil\frac{3.3k-1}{3}\big\rceil=3k$. Therefore, $\MP(G_k)\geq 3k$. Note that, diameter of $A_i$ is $2$ for each $i$. Therefore, any multipacking of $G_k$ can contain at most one vertex of $A_i$ for each $i$. So, $\MP(G_k)\leq 3k$. Hence $\MP(G_k)= 3k$.
\end{proof}


% \subsection{Proof of Lemma \ref{lem:mpfGk>=4k}}

% \begin{proof}

% \end{proof}















\noindent\textbf{Fractional multipacking: }
R. C. Brewster and  L. Duchesne \cite{brewster2013broadcast} introduced fractional multipacking in 2013 (also see \cite{teshima2014multipackings}).  Suppose $G$ is a graph with $V(G)=\{v_1,v_2,v_3,\dots,v_n\}$ and $w:V(G)\rightarrow [0,\infty)$  is a function. So, $w(v)$ is a weight on a vertex $v\in V(G)$. Let $w(S)=\sum_{u\in S}w(u)$ where $S\subseteq V(G)$.  We say   $w$ is a \textit{fractional multipacking} of $G$,  if $w( N_r[v])\leq r$ for each vertex $ v \in V(G) $ and for every integer $ r \geq 1 $. The \textit{fractional multipacking number} of $ G $ is the  value $\displaystyle \max_w w(V(G)) $ where $w$ is any fractional multipacking and it
	is denoted by $ \MP_f(G) $. A \textit{maximum fractional multipacking} is a fractional multipacking $w$  of a graph $ G $ such that	$ w(V(G))=\MP_f(G)$. If $w$ is a fractional multipacking, we define   a vector $y$ with the entries $y_j=w(v_j)$.  So,  \begin{center}
	    $\MP_f(G)=\max \{y.\mathbf{1} :  yA\leq c, y_{j}\geq 0\}.$
	\end{center} So, this is a  linear program which is the dual of the linear program   $\min \{c.x :  Ax\geq \mathbf{1}, x_{i,k}\geq 0\}$. Let,  
	    $\gamma_{b,f}(G)=\min \{c.x : Ax\geq \mathbf{1}, x_{i,k}\geq 0\}.$
	
 Using the strong duality theorem for linear programming, we can say that \begin{center}
     $\MP(G)\leq \MP_f(G)= \gamma_{b,f}(G)\leq \gamma_{b}(G).$
 \end{center}
 
 


% \begin{lemma}[$\ast$] \label{lem:mpfGk>=4k}
% If $k$ is a positive integer, then $ \MP_f(G_{k})\geq 4k$.
% \end{lemma}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{Figures/pentagon_frac.pdf}
    \caption{The $G_k$ graph with $\MP_f(G_k)=4k$.}
    \label{fig:pentagon_frac}
\end{figure}




\begin{lemma}  \label{lem:mpfGk=gammabGk=4k}
If $k$ is a positive integer, then $\MP_f(G_{k})=\gamma_b(G_{k})= 4k$.
\end{lemma}

\begin{proof}  
We define a function $w: V(G_k)\rightarrow [0,\infty)$  where $w(b_{i})=w(c_{i})=w(d_{i})=w(e_{i})=\frac{1}{3}$  for each $i=1,2,3,\dots,3k$ (Fig. \ref{fig:pentagon_frac}).  So, $w(G_k)=4k$. 
 We want to show that $w$ is a fractional multipacking of $G_{k}$. So, we have to prove that $w(N_r[v])\leq r$ for each vertex $ v \in V(G_{k}) $ and for every integer $ r \geq 1 $. We prove this statement using induction on $r$.	It can be checked that $w(N_r[v])\leq r$ for each vertex $ v \in V(G_{k}) $ and for each  $ r \in \{1,2,3,4\} $. Now assume that the statement is true for $r=s$, we want to prove that it is true for $r=s+4$. Observe that, $w(N_{s+4}[v]\setminus N_{s}[v])\leq 4$, $\forall v\in V(G_{k})$. Therefore,  $w(N_{s+4}[v])\leq w(N_{s}[v])+4\leq s+4$. So, the statement is true. So, $w$ is a fractional multipacking of $G_{k}$. Therefore, $\MP_f(G_{k})\geq 4k$.


Define a broadcast ${f}$ on $G_k$ as ${f}(v)=
    \begin{cases}
        4 & \text{if } v=a_i  \text{ and } i\equiv 2 \text{ (mod $3$)}  \\
        0 & \text{otherwise }
    \end{cases}$.\\
Here  ${f}$ is an efficient dominating broadcast and $\sum_{v\in V(G_k)}{f}(v)=4k$. So, $\gamma_b(G_k)\leq 4k$, for all $ k\in \mathbb{N}$. So, by the strong duality theorem  we have  $4k\leq \MP_f(G_k)= \gamma_{b,f}(G_k)\leq \gamma_{b}(G_k)\leq 4k$. Therefore, $\MP_f(G_{k})=\gamma_b(G_{k})= 4k$.  
\end{proof}



Lemma \ref{lem:mpGk=3k}  and  Lemma \ref{lem:mpfGk=gammabGk=4k} imply the following results.

\multipackingbroadcastgapecactus*

% Theorem \ref{thm:3k4k} says that, for all positive integers $k$,  $\gamma_b(G_{k})-\MP(G_{k})=k$.  This proves the following corollary.



\gammabDIFFGmpGcactus*

% \vspace{-0.6 cm}

% \gammabGBYmpGcactus*

% % \vspace{-0.6 cm}


% \boundimprovement* 




\begin{corollary} \label{cor:mpfG-mpG}  The difference $\MP_f(G)-\MP(G)$ can be arbitrarily large for cactus graphs (and for AT-free graphs).
\end{corollary}



% \begin{proof}
%     We get $\MP_f(G_{k})=4k$ by Lemma \ref{lem:mpfGk=gammabGk=4k} and  $\MP(G_{k})=3k$ by Lemma \ref{lem:mpGk=3k}. Therefore,   $\MP_f(G_{k})-\MP(G_{k})=k$  for all positive integers $k$. \hfill $\square$
% \end{proof}




% \begin{corollary}  \label{cor:gammabG2k/mpG2k}
% For every integer $k \geq 1$, there is a cactus graph $G_{k}$ with $\MP(G_{k})=4k$,  $\frac{\MP_f(G_{k})}{\MP(G_{k})}=\frac{4}{3}$ and $\frac{\gamma_b(G_{k})}{\MP(G_{k})}=\frac{4}{3}$.
% \end{corollary}


\section{$1/2$ - hyperbolic graphs}\label{sec:1/2-Hyperbolic graphs}

In this section, we show that the family of graphs $G_k$ (Fig. \ref{fig:pentagon}) is $\frac{1}{2}$-hyperbolic using a characterization of $\frac{1}{2}$-hyperbolic graphs. Using this fact, we  show that the difference $ \gamma_{b}(G) -  \MP(G) $ can be arbitrarily large for $\frac{1}{2}$-hyperbolic graphs. 
If the length of a shortest path $P$ between two vertices $x$ and $y$ of a cycle $C$ of $G$ is  smaller than the distance between $x$ and $y$ measured along $C$, then $P$ is called a \textit{bridge} of $C$. In $G$, a cycle $C$ is called \textit{well-bridged}  if for any vertex $x \in C$ there exists a bridge from $x$ to some vertex of $C$ or if the two neighbors of $x$ from $C$ are adjacent.  


\begin{figure}[ht]
    \centering
    \includegraphics[height=5.5cm]{Figures/hyperbolic_forbidden_graphs.pdf}
    \caption{Forbidden isometric subgraphs for $\frac{1}{2}$-hyperbolic graphs} 
    \label{fig:hyperbolic_forbidden_graphs}
\end{figure}



\begin{theorem}[\cite{bandelt20031}] \label{thm:1/2-Hyperbolic_graphs_classification}
    A graph $G$ is $\frac{1}{2}$-hyperbolic if and only if all cycles $C_n$, $n \neq 5$, of $G$ are well-bridged and none of the graphs in Figure \ref{fig:hyperbolic_forbidden_graphs} occur as isometric subgraphs of $G$.
\end{theorem}

Theorem \ref{thm:1/2-Hyperbolic_graphs_classification} yields the following.


\begin{lemma}\label{lem:pentagon_half_hyperbolic}
    The family of graphs $G_k$ (Fig. \ref{fig:pentagon}) is $\frac{1}{2}$-hyperbolic.
    
\end{lemma}


Lemma \ref{lem:mpGk=3k}, Lemma \ref{lem:mpfGk=gammabGk=4k} and Lemma \ref{lem:pentagon_half_hyperbolic} imply the following theorem.


\hypermultipackingbroadcastgape*




\hypergammabDIFFGmpG*


% \hypergammabGBYmpG*


From Theorem \ref{thm:1/2-Hyperbolic_graphs} and Lemma \ref{lem:mpfGk=gammabGk=4k}, we have the following.

\begin{corollary} \label{cor:hyper_mpfG-mpG}  The difference $\MP_f(G)-\MP(G)$ can be arbitrarily large for $\frac{1}{2}$-hyperbolic graphs.
\end{corollary}
























\section{Conclusion}\label{sec:conclusion_cactus}



We have shown that the  bound $\gamma_b(G)\leq 2\MP(G)+3$ for general graphs $G$ can be improved to $\gamma_b(G)\leq \frac{3}{2}\MP(G)+\frac{11}{2}$ for cactus graphs. Additionally, we have given a $(\frac{3}{2} + o(1))$-factor approximation algorithm for the multipacking problem on cactus graphs. A natural direction for future research is to investigate whether a polynomial-time algorithm exists for finding a maximum multipacking on cactus graph.



It remains an interesting open problem to determine the best possible value of the expression $\lim_{\MP(G)\to \infty}$ $\sup\{\gamma_{b}(G)/\MP(G)\}$ for cactus graphs. Extending this investigation to other important graph classes could also yield valuable insights into the relationship between broadcast domination and multipacking numbers.


==> frontmatter/abstract.tex <==
 A \emph{multipacking} in an undirected
	graph $ G = (V, E) $ is a set $ M \subseteq V  $  such that for every vertex $ v \in V $ and for every integer $ r \geq 1 $, the
	ball of radius $ r $ around $ v $ contains at most $ r $ vertices of $ M $, that is, there are at most
	$ r $ vertices in $ M $ at a distance at most $ r $ from $ v $ in $ G $. The
	\textit{multipacking number} of $ G $ is the maximum cardinality of a multipacking of $ G $ and
	is denoted by $ \MP(G) $. The
	\textsc{Multipacking} problem asks whether a graph contains a multipacking of size at least $k$.

    For more than a decade, it remained an open question whether the \textsc{Multipacking} problem  is \textsc{NP-complete} or solvable in polynomial time. Whereas the problem is known to be polynomial-time solvable for certain graph classes (e.g., strongly chordal graphs, grids, etc). Foucaud, Gras, Perez, and Sikora~\cite{foucaud2021complexity} [\textit{Algorithmica} 2021] made a step towards solving the open question by showing that the \textsc{Multipacking} problem  is \textsc{NP-complete} for directed graphs and it is \textsc{W[1]-hard} when parameterized by the solution size. 

    We study the hardness of the \textsc{Multipacking} problem and we prove that the \textsc{Multipacking} problem is \textsc{NP-complete} for undirected graphs, which answers the open question. Moreover, it is \textsc{W[2]-hard} for undirected graphs when parameterized by the solution size. Furthermore, we have shown that the problem is \textsc{NP-complete} and \textsc{W[2]-hard} (when parameterized by the solution size) even for various subclasses: chordal, bipartite, and claw-free graphs. Whereas, it is \textsc{NP-complete} for regular, and CONV graphs. Additionally, the problem is \textsc{NP-complete} and \textsc{W[2]-hard} (when parameterized by the solution size) for chordal $\cap$ $\frac{1}{2}$-hyperbolic graphs, which is a superclass of strongly chordal graphs where the problem is polynomial-time solvable.  Moreover, we provide approximation algorithms for the \textsc{Multipacking} problem for cactus (an unbounded hyperbolic graph-class), chordal (a bounded hyperbolic graph-class) and $\delta$-hyperbolic graphs.


      For a graph $ G = (V, E) $ with diameter $ \diam(G) $, a function
	$ f : V \rightarrow \{0, 1, 2, . . . , \diam(G)\} $ is called a \emph{broadcast} on $ G $. For each
	vertex $ u \in V  $, if  there exists a vertex $ v $ in $ G $ (possibly, $ u = v $) such that $ f (v) > 0 $ and
	$ d(u, v) \leq f (v) $, then $ f $ is called a \emph{dominating broadcast} on $ G $.  The cost of the dominating broadcast $f$ is the quantity $ \sum_{v\in V}f(v) $. The minimum cost of a
	dominating broadcast is the \textit{broadcast domination number} of $G$, denoted by $ \gamma_{b}(G) $. We study the relationship between $\MP(G)$ and $\gamma_b(G)$ for cactus, chordal and $\delta$-hyperbolic graphs.

     An \emph{$r$-multipacking} in an undirected
	graph $ G = (V, E) $ is a set $ M \subseteq V  $  such that for every vertex $ v \in V $ and for every integer $s$, $1\leq s \leq r $, the
	ball of radius $ s $ around $ v $ contains at most $ s $ vertices of $ M $, that is, there are at most
	$ s $ vertices in $ M $ at a distance at most $ s $ from $ v $ in $ G $. The
	$r$-\textsc{Multipacking} problem asks whether a graph contains an $r$-multipacking of size at least $k$.    It is known that \textsc{$1$-Multipacking} problem is \textsc{NP-complete} for planar bipartite graphs of maximum degree $3$, and chordal graphs. We study the hardness of the \textsc{$r$-Multipacking} problem, for $r\geq 2$. We prove that, for $r\geq 2$, the \textsc{$r$-Multipacking} problem is \textsc{NP-complete} even for planar bipartite graphs with bounded degree. Furthermore, we have shown that the problem is \textsc{NP-complete} for bounded diameter chordal graphs and bounded diameter bipartite graphs.


 Further,  we study some variants of  \textsc{Multipacking} problem for geometric point sets with respect to their Euclidean distances. We show that, for a point set in $\mathbb{R}^2$, a maximum $1$-multipacking can be computed in polynomial time but computing a maximum $2$-multipacking is \textsc{NP-hard}. Further, we provide approximation and parameterized solutions to the $2$-multipacking problem.

 Next,  we study  the \textsc{Minimum dominating broadcast} problem for geometric point set in $\mathbb{R}^d$ where the pairwise distance between the points are measured in Euclidean metric. We present a polynomial time algorithm for solving the \textsc{Minimum dominating broadcast} problem on a point set in $\mathbb{R}^d$. We provide bounds of the broadcast domination  number using kissing number. Further, we prove tight upper and lower bounds of the broadcast domination  number of  point sets in $\mathbb{R}^2$.   





 % -------------------------------------------------------------------------------------


% A \emph{multipacking} in an undirected graph $ G = (V, E) $ is a set $ M \subseteq V  $  such that for every vertex $ v \in V $ and for every integer $ r \geq 1 $, the ball of radius $ r $ around $ v $ contains at most $ r $ vertices of $ M $, that is, there are at most $ r $ vertices in $ M $ at a distance at most $ r $ from $ v $ in $ G $. The \textit{multipacking number} of $ G $ is the maximum cardinality of a multipacking of $ G $. The \textsc{Multipacking} problem asks whether a graph contains a multipacking of size at least $k$. It remained an open question whether the \textsc{Multipacking} problem  is \textsc{NP-complete} or solvable in polynomial time. Whereas the problem is known to be polynomial-time solvable for certain graph classes (e.g., strongly chordal graphs, grids, etc).  We study the hardness of the \textsc{Multipacking} problem and we prove that the \textsc{Multipacking} problem is \textsc{NP-complete} for undirected graphs, which answers the open question. Moreover, it is \textsc{W[2]-hard} for undirected graphs when parameterized by the solution size. Furthermore, we have shown that the problem is \textsc{NP-complete} and \textsc{W[2]-hard} (when parameterized by the solution size) even for various subclasses. Further, we provide approximation algorithms for the \textsc{Multipacking} problem for cactus, chordal and $\delta$-hyperbolic graphs. Further, we studied computational hardness and algorithms for multipacking and broadcast domination problems in geometric domain.


==> frontmatter/authorlist.tex <==



\medskip \noindent Contents of Chapter \ref{chapter:grids} are part of a journal article published in Discrete Applied Mathematics (DAM). The following authors contributed to Chapter \ref{chapter:grids} : Sandip Das.

\medskip \noindent Contents of Chapter \ref{chapter:orientetd} are part of a journal article published in Theoretical Computer Science (TCS). The following authors contributed to Chapter \ref{chapter:orientetd}: Sandip Das, Uma kant Sahoo, and Sagnik Sen.


\medskip \noindent Contents of Chapter \ref{chapter:butterfly} are part of a paper published in the proceedings of CALDAM 2021. The following authors contributed to Chapter \ref{chapter:butterfly}: Sheikh Shakil Akhtar and Sandip Das.



%\medskip \noindent Contents of Chapter \ref{chapter:rectangle-overlap-dom} are part of a paper published in the proceedings of COCOON 2019. The following authors contributed to Chapter \ref{chapter:rectangle-overlap-dom}: Sandip Das and Joydeep Mukherjee.


%\medskip \noindent Contents of Chapter \ref{chapter:dom-string} are part of a paper published in the proceedings of WG 2019.  The following authors contributed to Chapter \ref{chapter:dom-string}: Sandip Das and Joydeep Mukherjee.


==> frontmatter/dedication.tex <==
% dedication text



\begin{center}
    \Large To my family
\end{center}


==> frontmatter/official_declaration.tex <==
\thispagestyle{plain}

\begin{center}
 \Large {\bf \uppercase{DECLARATION}}
\end{center}

\vspace{3\baselineskip}

\noindent
\begin{tabular}{l l}
\textbf{Thesis Title} & \parbox{12cm}{\ReportTitle}\\\\
\textbf{Author} & \textit {\firstAuthor} \\\\
\textbf{Supervisor} & \Supervisor
\end{tabular}

\vspace{0.5\baselineskip}
\hrule
\vspace{2\baselineskip}

\noindent
I declare that this \MakeTextLowercase{\RoportType} entitled \emph{\ReportTitle} is the result of my own work except as cited in the references. The \MakeTextLowercase{\RoportType} has not been accepted for any degree and is not concurrently submitted in candidature of any other degree.


\vspace{3\baselineskip}
\begin{flushright}
\begin{minipage}[c]{0.63\textwidth}
\centering
\hrule 
\vspace{0.5\baselineskip}
{\bf \firstAuthor\par} 
\flushleft{\Department \\
\University}
\end{minipage}
\end{flushright}
\noindent{\bf Date:} \reportSubmissionDate

\newpage
\thispagestyle{empty}
\null
\newpage

==> frontmatter/thanks.tex <==
% the acknowledgements section

% \section*{Acknowledgements}

I would like to begin by expressing my sincere gratitude to my thesis supervisor, Professor Sandip Das. He has been not only an excellent mentor but also a constant source of encouragement and support throughout my PhD journey. His friendly nature, availability, and the healthy work environment he provided have made my research experience both pleasant and enriching. I am especially grateful for the academic freedom he offered me — the liberty to choose my research topics and collaborators. His role as a friend, philosopher, and guide has been invaluable, and I have learned immensely from him. I hope to continue learning from him in the future as well.

I am also deeply thankful to Dr.~Bhaswar B.~Bhattacharya, Dr.~Joydeep Mukherjee, Dr.~Florent Foucaud, and Dr.~Bodhayan Roy for their guidance and insightful suggestions. Their support has played a significant role in shaping my research abilities, and I have gained much from interacting with them.

I would also like to thank Dr.~Swami Sarvottamananda, Dr.~Subir Ghosh, Dr.~Binay Bhattacharya, and Dr.~Sagnik Sen for their support and encouragement. Their advice and assistance have been extremely helpful in many ways.

I extend my heartfelt thanks to Dr.~Daniel Lokshtanov. I consider myself fortunate to have had the opportunity to engage in discussions with him.  I have learned many things from him, and his suggestions have helped me refine my ideas and improve my skills.

My sincere thanks also go to Dr.~Harmender Gahlawat and Dr.~Arun Kumar Das, who have helped me in numerous ways. As my seniors and fellow students under the same supervisor, they have always been approachable and supportive. Their friendly advice and insightful discussions have been invaluable. 



I am further thankful to all my co-authors, from whom I have learned immensely. In particular, I would like to thank Dr.~Sandip Das, Dr.~Daniel Lokshtanov, Dr.~Florent Foucaud, Dr.~Joydeep Mukherjee, Dr.~Bodhayan Roy, Dr.~Bhaswar B.~Bhattacharya, Dr.~Arun Kumar Das, Dr.~Harmender Gahlawat, Dr.~Dibyayan Chakraborty, Dr.~Sanchita Paul, Saumya Sen, Ritam M.~Mitra, and Sweta Das for their collaboration and support.

I am fortunate to be part of a research environment that includes Ritam M.~Mitra, Saumya Sen, Sweta Das, Sangita Saha, Tamojit Saha, Soura Sena Das, Basudeb Roy, and Aashirwad Mohapatra. Their presence has made the office atmosphere friendly, productive, and research-oriented. I have shared many enriching discussions with them. I also wish to thank  Dr.~Dibyayan Chakraborty, Dr.~Uma Kant Sahoo, Dr.~Subhadeep Ranjan Dev, and Dr.~Sanjana Dey for their support and companionship.

I feel incredibly privileged to have learned from outstanding teachers, including Dr.~Ansuman Banerjee, Dr.~Bhargab B.~Bhattacharya, Dr.~Arijit Bishnu, Dr.~Sourav Chakraborty, Dr.~Nabanita Das, Dr.~Arijit Ghosh, Dr.~Sasthi C.~Ghosh, Dr.~Krishnendu Mukhopadhyaya, Dr.~Subhas C.~Nandy, Dr.~Sasanka Roy, and Dr.~Susmita Sur-Kolay. Their teaching has shaped my academic journey profoundly.

I am also thankful to the reviewers of my thesis for their constructive feedback and valuable suggestions, which have greatly improved the quality and clarity of this thesis.

Finally, I express my deepest gratitude to my family for their unwavering support, patience, and encouragement. My parents, Sk Rabiul Islam and Mousumi Islam, have always inspired me to pursue my aspirations. My sister, Romana Islam, has supported me in countless ways during my PhD journey. Words cannot adequately express my appreciation for my family. I am also thankful to the rest of my family members and friends, even though I could not mention everyone here individually.


